AutoBotCatcher: Blockchain-based P2P Botnet Detection for the Internet of Things

In general, a botnet is a collection of compromised internet computers, controlled by attackers for malicious purposes. To increase attacks' success chance and resilience against defence mechanisms, modern botnets have often a decentralized P2P structure. Here, IoT devices are playing a critical role, becoming one of the major tools for malicious parties to perform attacks. Notable examples are DDoS attacks on Krebs on Security and DYN, which have been performed by IoT devices part of botnets. We take a first step towards detecting P2P botnets in IoT, by proposing AutoBotCatcher, whose design is driven by the consideration that bots of the same botnet frequently communicate with each other and form communities. As such, the purpose of AutoBotCatcher is to dynamically analyze communities of IoT devices, formed according to their network traffic flows, to detect botnets. AutoBotCatcher exploits a permissioned Byzantine Fault Tolerant (BFT) blockchain, as a state transition machine that allows collaboration of a set of pre-identified parties without trust, in order to perform collaborative and dynamic botnet detection by collecting and auditing IoT devices' network traffic flows as blockchain transactions. In this paper, we focus on the design of the AutoBotCatcher by first defining the blockchain structure underlying AutoBotCatcher, then discussing its components.

==> BACKUP.tex <==
\textbf{Related work.}
Recent methods of P2P botnets detection on the network level can be roughly divided into:
\begin{itemize}
\item (a) communication graph structure based methods,
\item (b) traffic signature based methods,
\item (c) group or community behavior based methods. Botgrep \cite{botgrepFindingP2PbotsWithStructuredGraphAnalysis} is a communication graph structure based botnet detection method, which can detect P2P botnets through localizing structured communication graphs. However, this method can only identify structured communication subgraphs, rather than ensure those subgraphs contain P2P botnets
\end{itemize}
 

-- On CIDS
-- On Blockchain for IoT security
-- ML for intrusion detection 
\cite{dlforMaliciousFlowDetect}...

\textbf{Discussion taken from \cite{botnetCommunicationPatternsSurvey}}: In \cite{DetectingP2PbotnetsNetworkBehavAnalysisML}  Saad et al used the above mentioned approach of extracting features from network traffic, training a machine learning algorithm with known data, and using the trained algorithm for detection botnets. The algorithms were trained with normal and botnet traffic. For evaluation, this procedure was used on five different machine learning techniques. The results compare the different algorithms according to training and classification speed, and detection performance. Saad et al. concluded that by using this simple approach it is possible to detect botnets with analyzing only the packet metadata. However, those detectors are neither capable of adapting to changes in network traffic nor able to detect novel botnets.

\textbf{Discussion taken from \cite{botnetCommunicationPatternsSurvey}}: Alauthaman et al. \cite{P2PBotnetBasedOnDecisionTreeAndAdaptiveMultilayerNN} extended this simple approach with adding a filtering step before the machine learning and adding an automated feature selection. This works by adding a ma- chine learning algorithm that is used for discarding features which have only a small influence on the result. Better results in detecting known botnets were achieved than in previous works, but the performance on unknown botnets was not considered.

\textbf{Discussion taken from \cite{botnetCommunicationPatternsSurvey}} The detectors mentioned above train the machine learning algorithms with normal traffic for the normal class and with observed botnet traffic for the anomalous class to achieve a high accuracy. This implies that only the botnets which were encountered during training and close relatives can be detected. Therefore, the above stated goal of detecting unknown botnets can not be achieved \cite{outsideTheClosedWorldOnUsingMLforNetIntrusionDetection}, [18].

-- \cite{selfAdaptiveDLforAnomalyDetection5GNetworks}: 





%\textbf{Modularity.} \cite{findingEvaluatingCommunityStructureInNetworks}
%A classical approach to generate good community partitions (that are well separated from each other) is using a quality function.
%Modularity is one of the most used quality functions, that measures the strength of division of a network into clusters by comparing proportion of links inside the community with a model, and ranges in between -1 and 1.
%As defined in \cite{staticCommunityDetectionAlgorithmsForEvolvingNetworks}, in case of weighted networks, modularity defined as follows:

%\begin{align}
%Q = \frac{1}{2m} \sum_{ij}^{} \Big[(A_{ij} - \frac{k_i k_j}{2m})\Big] \delta(C_i,C_j),
%\end{align} 



\iffalse
\subsection{Why blockchain?}
Despite being popular, blockchain technology is not a solution that is looking for a problem.
In fact, as discussed in \cite{doYouNeedABlockchain}. ....
.
First, dynamic community detection with Louvain method requires to have community structure of the last snapshot of the mutual contacts graph.
Second, multiple parties, such as different device vendors, security policy enforcement bodies etc, should cooperate for successful Botnet detection.
--- Because, seeing the big picture of the whole network, as local solutions have a *local/small/limited network* view.
Blockchain technology can help to achieve trust-free relation among different parties, 
We need to find that have the real value, and contribution to the field.
So that is crucial to have benefits on adoption of blockchain technology, rather than existing solutions.
...
...
The main motivation of using blockchain in graph based community detection is enabling dynamic community analysis (see Section \ref{sec:architecture} for details).
In fact, one of the main difficulties in performing dynamic community analysis is the absence of timestamped data \cite{communityDetectionInGraphs}.
\fi




%Given a dynamic network DG, a dynamic community DC is defined as a set of distinct (node, periods) pairs: DC = {(v1, P1), (v2, P2),..., (vn, Pn )}, with Pn = ((ts0,te0), (ts1,te1) ... ($ts_n,te_n$)), with $ts_{*}$ $\leq$ $te_{*}$. DCD aims to identify the set C of all dynamic communities in DG. The partitions described by C can be neat as well as overlapping.




%\textit{the main underlying problem when computing communities on different snapshots is to decide which community at time $t$ evolved has evolved into which community at time $t+1$. -by- Considering that communities may merge, split, appear, or disappear.} .....


%\textbf{Hajime} \cite{hajime}: is a malicious internet worm, dubbed Hajime, which targets embedded/IoT devices and spreads by scanning the public internet devices running Telnet servers with insecure default credentials. What makes Hajime unique is that it does not rely  on centralized malware distribution server(s), but instead communicates over a distributed/decentralized overlay network to receive configuration and software updates.



%In \cite{dontTalkDefaultOffNetworking}: we argue that device communications should be default-off and desired network communications must be explicitly enabled. \\
%-- Unlike traditional networked applications or devices like a web browser or PC, IoT applications and devices serve narrowly defined purposes and do not require access to all services in the network. \\
%-- Two factors make these IoT devices notorious weak links in network security; they are easy to compromise and and their compromise goes undetected (They present good examples on different compromised IoT devices on Toys, Mirai to VCR etc., can take the same examples). IoT devices are often low-margin products whose primary goal is convenience. They are often do not follow security best practices and, even if they do, may not be updatable when best practices change or bugs are discovered. \\
%-- Calm Computing \cite{calmComputing}: Following Mark Weiser's vision of 'Calm computing', IoT devices are intended to be unobtrusive and seamlessly helpful. As a result, owners interact with then infrequently and in very limited ways - \textit{how would you know if your thermostat was part of a botnet?} \\
%--Given that IoT devices are so easy to undetectably compromise, one might conclude that they represent an undebatable security threat. However, one property of the Internet of Things makes them easier to secure and to contain in the event of compromise. Unlike complex, application-rich end-user devices such as laptops and tablets,\textbf{ IoT devices have narrow, application-specific uses.} A thermostat, light bulb, or webcam does not act as a platform for scores of new networked applications each year. \textbf{Consequently, their communication patterns are also stable and predictable. A Nest thermostat talks only to Nest servers, while only a small number of clients connect to home webcams.}



%\textbf{AutoBotCatcher execution.} Execution of the AutoBotCatcher is as follows: agents sense network flow data of devices in their device subnet; agents form  network-data transactions and sends them to the transaction pool;  throughout a round, a block generator takes subset of transactions from the transaction pool to form a block; when the round ends block validators extracts the new version of the mutual contacts graph by using the previous snapshot of it recorded in the previous state of the blockchain; block generators perform Louvain community detection method by initializing it with the community set mapping (community set to device IP addresses) of the previous state for dynamic community detection;  for the same communities with the previous step, AutoBotCatcher checks perturbations in the communities such as newly added devices and records IP addresses part of the botnet communities; for newly emerged communities, AutoBotCatcher perform botnet community detection method, marks botnet communities and records IP addresses part of botnet communities; finally AutoBotCatcher generates and sends blacklist transactions to all agents, that includes blacklisted IP addresses part of botnets. 





--------------------
--------------------
--------------------
----------------------------------------
--- problem statement--------------------
----------------------------------------
--------------------
--------------------
--------------------





%\cite{aP2PCollaborativeIDS}
%\textit{We are given a set of intrusion detection systems D = \{{$d_{i}\mid$i = 1, 2, . . . , m}\}, where each detection system $d_{i}$ monitors a corresponding sub-network $sn_{i}$ that is connected to the Internet. Each detection system $d_{i}$ monitors the traffic to/from its subnetwork $sn_{i}$ , in order to gather evidence of potentially suspicious activity. Each of these intrusion detection systems become peers in a peer-to-peer system that forms the collaborative intrusion detection system. Periodically, each detection system shares evidence about the suspicious activity that it has seen on its subnetwork.
%The evidence that is shared can potentially take many forms. In this paper, we consider the case where the evidence to be shared is a set of suspicious source IP addresses that have been sending traffic to the monitored subnetwork. We refer to the set of suspicious source IP addresses that have been observed by detection system $d_{i}$ as its blacklist $b_{i}$ =  \{ {$s_{ij}$ $\epsilon$ IP$\mid$j =1, 2, . . . , $n_{i}$}\}, where $s_{ij}$ is the $j^{th}$ source address that has been sending suspicious traffic to subnetwork $sn_{i}$.} 




%To this end, agents continuously monitor connections of IoT devices in their subnet, and gather meta-data information (such as packet sizes, IP addresses) about their network traffic flows in form of blockchain transactions (see Definition \ref{def:NFT}).
%Block generators use  network traffic flow meta-data information collected by agents to model mutual contact information of all IoT devices and other hosts in the network.
%Particularly, block generators model mutual contact information, that is represented as  mutual contact graphs (see Section \ref{sec:mutualContacts}).% from all IoT devices and other hosts in the network.
%Periodically, block generators: update mutual contacts information with new network flow meta-data information sent by agents; perform botnet community detection on mutual contact information dynamically; and inform agents about IoT devices and hosts that are part of a botnet (see Section \ref{sec:architecture}). 



%Moreover, botnets tend to hide their operation \cite{botnetCommunicationPatternsSurvey}, aka act \textit{stealthy}, to increase success chance of attacks as malicious activities may not be observable.



------------ ------------
------------introduction------------
------------ ------------
%Moreover, botnets tend to hide their operation \cite{botnetCommunicationPatternsSurvey}, aka act \textit{stealthy}, to increase success chance of attacks as malicious activities may not be observable.
%Anti-signature stealth entails the capability of manipulating the characteristics of bot-generated traffic to mask features that could be observed by signature-based detectors




%In designing AutoBotCatcher, we assume the presence of gateway devices, such as Dell Edge Gateways\footnote{$dell.com/us/business/p/edge-gateway$}, deployed in the network boundaries, where IoT devices communicate directly through gateways. 
%AutoBotCathcer's execution starts with operation of gateway devices in network boundaries, referred to as \textit{agents}.  Particularly, agents monitor network traffic flow of IoT devices and take actions, such as: generating network-flow transactions (NFTs) (see Definition \ref{def:NFT}) and forcing infected devices to shut down. 




\iffalse
Dynamic community. The network structure that AutoBotCatcher is a \textit{dynamic network}, as network evolves with the time due to addition and removal of IoT devices. 
%BC1604 check english in the above sentence 
%GOKHAN: Deprecated.
This causes mutations of communities, referred to as \textit{dynamic communities}. 
Therefore, in AutoBotCatcher, we treat IoT device communities, benign or botnet, as dynamic communities.
To this end, AutoBotCatcher tracks differences in identified communities, and perform botnet detection dynamically (see Section \ref{sec:architecture}).
\fi


%\textbf{MERGE, FROM INTRODUCTION 9th para}
%\textit{Bots have dynamical communication behaviors \cite{peercleanUnveilingP2PbotnetsThroughDynamicGroupBehaviorAnalysis}, thus it is not practical to detect a single bot \cite{peerhunter}.
%On the other hand, as presented in \cite{friendsOfAnEnemyMutualContacts}, P2P bots in a network communicate with at least one mutual peer outside the network with a high probability.
%Given that, AutoBotCatcher dynamically performs community behaviour analysis on snapshots of the evolving mutual contacts graph.
%To this end, we define a new BFT blockchain paradigm for AutoBotCatcher, where \textit{state} of the blockchain consists of snapshot of the mutual contacts graph (see Section \ref{sec:paradigm}).
%}


\textbf{Assumptions.}
--- We assume the presence of gateway devices, such as Dell Edge Gateways\footnote{$dell.com/us/business/p/edge-gateway$}, deployed in the network boundaries  to  monitor network traffic flow of a group of IoT devices, called \textit{subnet};
--- IoT devices communicate directly through gateways;%, and there are no side-channels.
--- Gateways are trusted. As such, we assume they behave as expected, and can not be compromised and act maliciously.



To achieve long-term control, a bot must be stealthy during every part of its lifecycle, unlike its predecessors. As a result, most bots have a relatively small network footprint and do not create much traffic during typical operation. Once a bot is in place, the only required traffic consists of incoming commands and outgoing responses, constituting the botnet’s command and control (C \& C) channel.



--------------------
-------------------BACKGROUND-------------
-------------------
%Bots of a P2P botnet communicate with at least one mutual contact with very high probability \cite{friendsOfAnEnemyMutualContacts,peerhunter}.
%Mutual contacts are shared connections between a pair of IoT devices and/or other hosts.
%For example, let us assume \textit{Host A}\footnote{Here, \textit{Host} refers to both IoT devices and other hosts in the network} is connected to \textit{Host C}; given that, if \textit{Host B} is also connected to \textit{Host C}; then \textit{Host A} and \textit{Host B} share a mutual contact, that is \textit{Host C}.
%Mutual contacts can be exploited for botnet detection \cite{friendsOfAnEnemyMutualContacts}.


\subsection{Intrusion Detection Systems (CIDS)}
\textbf{Intrusion Detection - Taken From \cite{intrusionDetectionMeetsBlockchainTechnology}} Intrusion detection describes the process of monitoring network or system events for any sign of possible incidents. An IDS is an application to realize the process of intrusion detection. Basically, an IDS can provide two main functions:
\begin{itemize}
\item Information Recording: An IDS can monitor the target objects and record information locally. Then, the collected data can be sent to other facilities for analysis, like a central event management system.
\item Alert Generation: The main task of an IDS is to generate alerts (alarms) to inform security administrators of important identified anomalies. False alarm rates are
an important measurement to decide whether an IDS is effective or not.
\end{itemize}
As mentioned, an IDS can be generally classified into Host-based IDS (HIDS) and Network-based IDS (NIDS).

--For us relevant one is NIDS.

\textbf{NIDS - Types - Taken from \cite{outsideTheClosedWorldOnUsingMLforNetIntrusionDetection} (Cok iyi degil...)}: 
Traditionally, network intrusion detection systems (NIDS) are broadly classified based on the style of detection they are using: systems relying on misuse-detection monitor activity with precise descriptions of known malicious behavior, while anomaly-detection systems have a notion of normal activity and flag deviations from that profile. Other styles include specification-based and behavioral detection. These approaches focus respectively on defining allowed types of activity in order to flag any other activity as forbidden, and analyzing patterns of activity and surrounding context to find secondary evidence of attacks.


-- Based on the detection approaches, an IDS can be either a signature-based or an anomaly-based system \textbf{Taken From \cite{intrusionDetectionMeetsBlockchainTechnology}}:
\begin{itemize}
\item The signature-based detection method, also called misuse-based detection, is usually effective in detecting known exploits but would be ineffective for unseen threats and the variants of known threats.
\item The anomaly-based detection has the capability of detecting unknown threats (or zero-day threats). Such detection firstly establishes a normal profile by monitoring the system or network events for a period of time, and then identifies any behavior that would be significantly different from the established profiles
\end{itemize}


\subsection{Collaborative IDS}
\textbf{Taken From \cite{intrusionDetectionMeetsBlockchainTechnology}:}
CIDSs were developed in practice, with the purpose of enhancing the performance of a single IDS, which may be easily bypassed by advanced or complicated attacks like denial-of-service (DoS) attack.


\subsection{Blockchain Technology}
A promising decentralized platform for IoT is blockchain. Blockchain is the concept of a distributed ledger maintained by a peer-to-peer network. Its data structure consists of bundled data chunks called blocks and peers in a blockchain broadcast blocks by exploiting public-key cryptography. Blocks are recorded in the blockchain with exact ordering. Briefly, a block contains: a set of transactions (exchange and transfer of information); a timestamp; a reference to the preceding block that identifies the block's place in the blockchain; an authenticated data structure (e.g., a merkle tree \cite{merkle}) to ensure block integrity.\footnote{Block structure varies in different blockchain protocols, here we list the most common elements.} Modern blockchain protocols, such as Ethereum\footnote{ethereum.org}, possess scripting systems that allow the coding and execution of computing programs on the blockchain itself, referred to as smart contracts. \cite{blockchainSurvey} Different blockchain protocols may employ different methodologies to achieve consensus. For example, some blockchains use \textit{Proof of Work (PoW)} \cite{bitcoinNakamoto}, while others  \textit{Byzantine Fault Tolerant (BFT)} \cite{tendermint}. In PoW blockchains, peers, referred to as block miners, have to have to use their hardware resources and energy  to solve a cryptographic puzzle as proof of their work, in order to be authorized to generate a new block. Notably, PoW blockchains are able to maintain a relative low throughput while scaling to thousands of nodes in achieving consensus, while BFT blockchains can maintain a relative high throughput with only few nodes. Other consensus protocols are emerging, for example Proof Of Stake (PoS) \cite{blockchainSurvey}, but for the scope of this work we consider mature and well implemented protocols like PoW and BFT.

\textbf{Blockchain structure.} 
Transactions transfer information (i.e. data packets) between peers and they have unique identifiers, input data, and they are bundled into data chunks called blocks. 
Every block contains set of transactions, a timestamp, a reference to the preceding block, and an authenticated data structure (i.e. a merkle tree) from previous transactions, and forms the blockchain. 
Blockchains are peer to peer networks, and nodes are connected to other nodes as peers to share transactions and blocks. 
A copy of the blockchain is stored on every node in the network and these peers exchange the latest block information with each other to ensure that all of them have the same shared database.



\subsection{Machine Learning Anomaly Detection}
\textbf{Definition Machine Learning in \cite{botnetCommunicationPatternsSurvey}}:  Machine learning is a process which modifies the parameters of an algorithm until the algorithm output matches the expected output for given inputs. This is called training. A trained machine learning algorithm can be an approximation of the dependencies between the trained parameters and the expected results. 


\textbf{About Machine Learning: from \cite{fewUsefulThingsToKnowAboutML}}
Machine learning algorithms can figure out how to perform important tasks by generalizing from experiments. 
Many different types of machine learning exist, the most mature and widely used one is \textit{classification}. A classifier is a system that inputs (typically) a vector of discrete and/or continuous \textit{feature} values and outputs a single discrete value, the \textit{class}. \\
-- Easily the most important factor of machine learning algorithm to succeed is the features used. If you have many independent features that each correlate well with the
class, learning is easy. In parallel, in \cite{mlForEncryptedMAlwareTrafClassification}, authors stated that properly done feature engineering by domain experts and choice of feautes has a much greater effect on the performance. 


\textbf{Anomaly detection \cite{outsideTheClosedWorldOnUsingMLforNetIntrusionDetection}}: Anomaly detection systems find deviations from \textit{expected behavior}. Based on a notion of \textit{normal activity}, they report deviations from that profile as alerts. The basic assumption underlying any anomaly detection system — malicious activity exhibits characteristics not observed for normal usage — was first introduced by Denning in her seminal work on
the host-based IDES system \cite{intrusionDetectionModelFirst1987} in 1987.  To capture normal activity, IDES (and its successor NIDES) used a combination of statistical metrics and profiles. Since then, many more approaches have been pursued. Often, they borrow schemes from the machine learning community, such as information theory, neural networks, support vector
machines, genetic algorithms, artificial immune systems, and many more. 



\subsection{Motivation}

\textbf{Relevance of the blockchain.}

\textbf{Difficulty of P2P botnets.}


\textbf{Why community behavior detection?}
\cite{theBotnetProblem}Botnets are built on the very premise of extending the attacker’s control over his victims. To achieve long-term control, a bot must be stealthy during every part of its lifecycle, unlike its predecessors. As a result, most bots have a relatively small network footprint and do not create much traffic during typical operation. Once a bot is in place, the only required traffic consists of incoming commands and outgoing responses, constituting the botnet’s command and control (C \& C) channel \cite{theBotnetProblem}. 



---  PRIVACY IMPLICATIONS ----
\iffalse
In \cite{privacyImplicationsCyberSecSystemsSurvey}: Classification of cyber-security systems: 1) according to system architecture as \textit{standalone}, \textit{centralized client-server}, and \textbf{\textit{collaborative}}: 2) Type of detection as \textbf{\textit{anomaly-based detection}} and \textit{signature based detection}; 3) Type of data as \textit{application data}, \textit{file data}, and \textbf{\textit{network data}}; 4) Ecosystems as \textit{enterprise}, \textit{mobile devices}, and \textbf{\textit{IoT}}.

-- Privacy implications from \cite{privacyImplicationsCyberSecSystemsSurvey}:
\begin{itemize}
\item \textbf{Collaborative}: \textit{(Data Exposure)} High network centricity. Check data in transit and data at rest/use protection for sharing users.  
\item \textbf{Anomaly-based detection}: \textit{(Identification and Sensitivity)} Re-identifying and sensitive data accessed during training and monitoring. Check specific data and degree of re-identifiability/sensitivity.\\
\textit{(Frequency of Release)} Check risk of correlation
between multiple releases used to update the model
\item \textbf{Ecosystem IoT}: \textit{(Identification)} Check for re-identifying data (e.g., video from cameras). \\
\textit{(Sensitivity)} Check for access to sensible data on medical conditions, behavioral data. \\
\textit{Data exposure} Check architecture (Gateway, cloud) and its risks.
\item \textbf{Network:} 
	\begin{itemize}
		\item \textbf{IP Packet Header:} \textit{(Identification)} Re-identifiable (e.g., by static IP address in organizations, geo-location, organizational affiliation). Estimate risk. \\
        \textit{(Sensitivity)} Revealed sensible data includes sender/receiver hosts (visited websites).
		\item \textbf{IP Packet Header + Content:} \textit{(Identification)} Re-identifiable (e.g., through IP, username, email). Estimate risk. \\
        \textit{(Sensitivity)} Revealed sensible data includes sender/receiver hosts, communication content.
	\end{itemize}
\end{itemize}
\fi


-----------------------------------------------------------
	----------------------SYSTEM----------------------
-----------------------------------------------------------
%\cite{peerhunter}: "We consider a botnet community as a group of compromised machines that communicate with each other or connect to the same set of botmasters through the same C\&C channel, are controlled by the same attacker, and aim to perform similar malicious activities."
%d  : 3) Threat model.
%\textbf{Threat model.}
%In designing a botnet detection and prevention mechanism, threat model should be clearly identified.  At this purpose, let us define, in the following, the threat model that we deal in this work; \\
%$\diamond$ Botmasters encrypt C\&C channels, and therefore deep-packet-inspection (DPI) techniques are not suitable;\\
%$\diamond$ IoT devices can become part of a botnet anytime;\\
%$\diamond$ Botnets tend to hide their operations and botmasters try to stay as stealthy as possible \cite{botnetCommunicationPatternsSurvey}. As such, we assume that botnets are able to manipulate characteristics of bot traffic, and thus they are able to make network flow traffic signature based defense approaches incompetent;   %which makes traffic signature based  thus ; 
%BC1604 it seems something is missing....by acting.?\\
%GOKHAN: Fixed, rewritten.
%$\diamond$ Botnets are in their waiting stage, where bots are joined to the C\&C network and wait for commands from the botmaster, thus their malicious activity may not be easily observable.
%AutoBotCatcher performs P2P botnet detection in IoT dynamically and collaboratively with by exploiting blockchain technology.
%As defence strategies against botnets evolve and improve, botmasters also change their strategies to increase success chance of attacks performed by their botnets.






















--- BOT DEFINITION ----

\iffalse
\begin{itemize}
\item Bots (also called zombies \cite{securityGlossary}) are infected machines that execute the bot executable. Those machines process the tasks supplied by the C\&C server.
\item The C\&C server is the central rallying point for the botnet. Since this server is capable of controlling every bot, it has to be protected from takeover by third-parties like, e.g., law enforcement, researchers, or rivaling bot masters. Modern botnet topologies (e.g., Peer to Peer (P2P)) can utilize regular bots that are part of the botnet as C\&C server. Thus, the threat of bringing down the botnet via a single point of failure is remedied.
\item The botmaster is the person controlling the botnet via the C\&C server. Botmasters try to stay as stealthy as possible, because unmasking the identity of the botmaster can lead to potential prosecution. This can be achieved for example by using as little traffic as possible, or by not using a direct connection to the rest of the botnet.
\end{itemize}
-- Since botnets tend to hide their operation, detection of botnets is an active field of research. Botnet detection can target one of the three parts of a botnet. \\
-- A communication pattern is a sequence of exchanged messages needed for a specific communication scenario. \\
-- Since network communication is paramount for a botnet, it has to be present and can therefore be used for bot detection. This is called network-based bot detection. \\
-- The least complex approach for implementing a network- based detector is signature-based detection or syntactic detection \cite{taxonomyBotnet}. Such detector can be rather easily by-passed by an attacker by: 1) modifying the used C\&C commands, 2)adding random sequences at the beginning or at arbitrary positions of a C\&C command (called padding), and 3) protocol encryption can thwart every signature-based detection. \\
-- Behavioral network analysis can be used to overcome this limitation. This technique relies on classifying network traffic as either normal traffic or anomalous traffic \cite{taxonomyBotnet}. Therefore, this technique is also called network anomaly detection. \\
\begin{itemize}
\item One way to build a network anomaly detector is to observe “abnormal” behavior (e.g., botnet C\&C traffic) and to find characteristic patterns or properties (e.g., packet timing, packet count, packet length). These properties are called features. The same can be achieved by observing “normal” behavior (i.e., legitimate traffic captured during network operation), extracting features, and defining network traffic that does not match these patterns as an anomaly.
\item No inspection of the payload is needed, and therefore this approach works with encrypted or obfuscated network traffic. Since this technique tries to find generalized properties of unwanted traffic, it can theoretically be used to detect previously unknown botnets. A simple way to implement this procedure is to use machine learning.
\item  Since there is not necessarily an underlying correlation in the data, the results have to be validated and used with caution.
\end{itemize}
\fi





--- Booters ---
%DDoS-for-hire services, also known as \textit{booters}, have commoditized DDoS attacks and enabled abusive subscribers of these services to cheaply extort, harass and intimidate businesses and people by knocking them offline. These services are operated by profit-motivated adversaries that have scaled up their DDoS infrastructure to meet the increasing demand for DDoS attacks. They have commoditized DDoS attacks that reach upwards of 2-3 Gbps. By offering a low-cost shared DDoS attack infrastructure, these criminal support services have attracted thousands of malicious customers and are responsible for hundreds of thousands of DDoS attacks a year.







------------------------------------------------------
	-----------------PARADIGM------------------
------------------------------------------------------
$NT_{x}$ = ($Device_{addr} HF(IP_{src}), HF(IP_{dest}), Tx-Pool_{addr}$) is a tuple, where $Device_{addr}$  presents the unique public key of the device that sends the transaction ; $HF(IP_{src})$ and $HF(IP_{dest})$ present hashes of the source and destination IP addresses of network traffic flow, where HF is the hash function; $PS$ represents size of the network packet (in bytes); $Prt$ represents protocol type of the packet (i.e. TCP or UDP), and $Tx-Pool_{addr}$ presents public key of the transaction pool. 

Blockchain paradigm presents an integrity focused approach to achieve consensus among different parties on timestamped data, which are shared as \textit{transactions}, with the assumption of byzantine behaviors of parties.




\footnote{We note that, our definition on mutual contracts graph can be easily modeled as a standard smart contract concept\cite{szabo} of second generation blockchains such as Ethereum or Hyperledger, by exploiting key-value storages to store vertice addresses (Host IPS) as keys and their weights as values; and by applying the mutual contact graph extraction algorithm as smart contract code. This is a advantage of usability and adaptability of the proposed blockchain notation, as it does not requires to implement a new blockchain protocol, rather can be easily adaptable to widely adopted protocols.} 





Obfuscation
%In order to protect the privacy of different parties participating in AutoBotCatcher, we assume that agent obfuscates IP addresses of IoT devices before inserting their collected meta-data into  transactions.  
%Here, we assume that, obfuscation performed by agents result with a unique and collision-free value for all IoT devices.
%Particularly, that can be done by a function such as SHA256, in oder to hash IP address and global MAC addresses of IoT devices with a hash function.
%By this way, privacy of the parties collaborating in botnet detection is protected, since: block generators only deal with obfuscated values; and agents can only decode able to solve/understand







--------------------------------------------------------
 ------------------------intro------------------------
--------------------------------------------------------
%snapshots are periodically generated as mutual contact information of IoT devices evolve over time. 
%In this way, unlike other community and group behaviour based botnet detection mechanisms, AutoBotCatcher is able adapt to evolving networks, and thus can detect emerging botnets.
%AutoBotCatcher consists of seven modules to perform botnet community detection and take preventive measure against spread of the botnets (see Section \ref{sec:architecture}). 




%\textbf{Botnet detection in IoT.}
%Due to rise of compromises in IoT domain, literature offer many works dealing with botnet detection in IoT domain.  
%Many works on IoT domain employed machine learning techniques in order to monitor network anomalies and detect botnets .


%In what follows, we discuss the related work on Botnet detection by classifying them into two groups: first we discuss botnet detection methodologies proposed for IoT domain; and second, we discuss various interesting botnet detection methodologies proposed for another domain that deserve to be cited and com- pared to our solution.



In the literature, a system’s a attack surface has been formally defined as the “subset of the system’s resources (methods, channels, and data) that can be potentially used by an a attacker to launch an a attack.”
Continuously reshaping a system’s attack surface increases complexity and cost for malicious actors, forcing them to continuously reassess their cyber operations.


--------------------------------------------------------------------------------------
------------------------------------RELATED WORK--------------------------------------
--------------------------------------------------------------------------------------



%done : 1)intro
\textbf{Related Work}%\label{sec:related}
In recent years, vast amounts of work has been proposed as P2P botnet detection solutions. Mainly, botnet detection methodologies can be categorized into two groups: host-based and network-based approaches.  Host-based approaches require individual monitoring for all hosts, which is impractical for IoT domain. Therefore, we focus on network-based approaches which we classify into two groups.

-- \textit{Network traffic signature based approaches.} Literature offers many works that utilize network traffic behaviour classification for host, such in order to identify whether they are benign or malicious, such as \cite{scalableSystemForStealthyP2PbotnetDetection, peershark}.
For example, in \cite{scalableSystemForStealthyP2PbotnetDetection}, a statistical network traffic fingerprinting approach that is using unsupervised machine learning techniques to identify P2P activity and to group hosts participate in malicious P2P traffic.
However in a dynamic network, such approaches are ineffective, as botnets can randomize their traffic, thus traffic signature will vary. 
Some other works based on network traffic signatures rely on deep packet inspection techniques (DPI) in order to identify P2P botnets, such as \cite{botminer, botdetector}. 
%For example, BotMiner proposed in \cite{botminer}, groups hosts that share similar communication patterns in performing malicious activities.
For example, BotDetector proposed in \cite{botdetector},  leverages on DPI techniques to monitor information recorded on HTTP headers is proposed.
However, DPI based approaches are computationally expensive, and traffic flow encryption makes them methods ineffective.


-- \textit{Group and community behavior based approaches.} Similar to AutoBotCatcher, some works in the literature uses group and community behaviours to detect botnets \cite{friendsOfAnEnemyMutualContacts,peercleanUnveilingP2PbotnetsThroughDynamicGroupBehaviorAnalysis,peerhunter}.
For example, in \cite{friendsOfAnEnemyMutualContacts}, a mutual contacts based approach that is based on network traffic flow of hosts is proposed to identify bots in a P2P network. However, this approach requires bot seeds/discovered bots in order to identify bots, which may not be available. 
Moreover, this approach is only limited to detect bots from previously known bot types.
%PeerClean proposed in \cite{peercleanUnveilingP2PbotnetsThroughDynamicGroupBehaviorAnalysis}, performs group level behavior analysis on network flow traffic with SVM method. Similarly to the previous work, this approach is only limited to known bot types.
More recently, in \cite{peerhunter}, a network flow level community behaviour analysis is performed for P2P botnet detection.
Similar to our proposal, also this approach performs community analysis approach based on mutual contacts graph have been proposed.
However, it is a static approach, as it performs botnet detection once on collected network flow traffic data, yet AutoBotCatcher dynamically performs botnet detection on successive snapshots of the mutual contacts graph with the help of blockchain technology. 


%discussed in what follows.


% : 2) Network traffic signature based
\textbf{Network traffic signature based approaches.} Literature offers many works that utilize network traffic behaviour classification for hosts, in order to identify whether they are benign or malicious, such as \cite{scalableSystemForStealthyP2PbotnetDetection, peershark, botminer, botdetector}.   In \cite{scalableSystemForStealthyP2PbotnetDetection}, a statistical network traffic fingerprinting approach that is using unsupervised machine learning techniques to identify P2P activity and to group hosts participate in malicious P2P traffic. PeerSark, proposed in \cite{peershark}, a port and protocol oblivious conversation-based approach to detect P2P botnet traffic is proposed. %NO DPI. However in a dynamic network, such approaches are ineffective, as botnets can randomize their traffic, thus traffic signature will vary. 

%DPI-based traffic signature approaches.
Some other works rely on deep packet inspection techniques (DPI) in order to identify P2P botnets. 
For example, BotMiner proposed in \cite{botminer}, groups hosts that share similar communication patterns in performing malicious activities.
More recently, BotDetector proposed in \cite{botdetector},  leverages on DPI techniques to monitor information recorded on HTTP headers is proposed.
However, DPI based approaches are computationally expensive, and traffic flow encryption makes them methods ineffective.



% : 3) group and community behavior based
\textbf{Group and community behavior based approaches.}
In \cite{friendsOfAnEnemyMutualContacts}, a mutual contacts based approach that is based on network traffic flow of hosts is proposed to identify bots in a P2P network. However, this approach requires bot seeds/discovered bots in order to identify bots, which may not be available. 
Moreover, this approach is only limited to detect bots from previously known bot types.
PeerClean proposed in \cite{peercleanUnveilingP2PbotnetsThroughDynamicGroupBehaviorAnalysis}, performs group level behavior analysis on network flow traffic with SVM method. Similarly to the previous work, this approach is only limited to known bot types.
More recently, in \cite{peerhunter}, a network flow level community behaviour analysis is performed for P2P botnet detection.
Similar to our proposal, also this approach performs community analysis approach based on mutual contacts graph have been proposed.
However, it is a static approach, as it performs botnet detection once on collected network flow traffic data, yet AutoBotCatcher dynamically performs botnet detection on successive snapshots of the mutual contacts graph with the help of blockchain technology. 
%Moreover, it does not take any prevention measurements like AutoBotCatcher. 

%\textbf{-- Total number of citation can be reduced like 15}
%\textbf{-- Related work can be moved to introduction. }


% : 3) graph-based
%BOTGREP
%In \cite{botgrepFindingP2PbotsWithStructuredGraphAnalysis}, a communication graph structure based approach for P2P botnet detection.....
%. Botgrep [18] is a communication graph structure based botnet detection method, which can detect P2P botnets through localizing structured communication graphs. However, this method can only identify structured communication subgraphs, rather than ensure those subgraphs contain P2P botnets}

==> DEPRECATED.tex <==
As per Section \ref{sec:architecture}, light peer devices send transactions to full peer devices, and those will include them in the newly generated blocks.
Hence, the first type of experiment that we run to test performance is a stress test, in which a full peer device DoSed by twenty light peer devices that are continuously sending transactions to it (see Section \ref{sec:perfEva1}).
Then, we shift the focus to the generation of sub-blockchains that contain different number of full peer devices.
In that, we monitor performance and resource usage of the full peer devices in different sized sub-blockchains (see Section \ref{sec:perfEva2}).




\begin{figure*} 
    \centering
   \subfloat[Perf Eva \rom{1}: CPU Light peer device]{%
     \includegraphics[width=0.5\linewidth]{figures/LightCPU.png}}
     \label{1a} \hfill
  \subfloat[Perf Eva \rom{1}: CPU Full peer device]{%
      \includegraphics[width=0.5\linewidth]{figures/20LiDOS.png}}
     \label{1b} \hfill
  \subfloat[Perf Eva \rom{2}: CPU usage in Emulation \rom{1}]{%      
     \includegraphics[width=0.33\linewidth]{figures/20liYeni.png}}
  	  \label{1c}
  \subfloat[Perf Eva \rom{2}: CPU usage in Emulation \rom{2}]{%
      \includegraphics[width=0.33\linewidth]{figures/40liYeni.png}}
    \label{1d}\hfill
  \subfloat[Perf Eva \rom{2}: CPU usage in Emulation \rom{3}]{%
      \includegraphics[width=0.33\linewidth]{figures/100luYeni.png}}
     \label{1e}\hfill
  \subfloat[Perf Eva \rom{2}: CPU usage in Emulation \rom{4}]{%
      \includegraphics[width=0.33\linewidth]{figures/200luYeni.png}}
     \label{1f} 
  \caption{CPU utilization of devices in Performance Evaluation \rom{1} and \rom{2}}
  \label{fig:CpuUtil} 
\end{figure*}





ARCHITECTURE
8 MARCH DEPRECATED:
%The key challenge for successful integration is the limited transaction throughputs of PoW-based blockchains.
%In fact, the more devices become blockchain peers, the higher transaction throughput must be achieved.
%Hybrid-IoT achieves high ratio of the transaction throughput to number of devices by having multiple PoW-based sub-blockchains generated according to sweet-spot settings defined in Section \ref{sec:sweetspot}.
%Sub-blockchains have to be connected to each other in order to achieve interoperability.
%
%Particularly, full peer devices include inter-blockchain transactions to the newly generated blocks in their sub-blockchain.
%Then, inter-blockchain transactions transferred to the one node of the BFT-based blockchain connector framework that is assigned for its sub-blockchain.
%
%High transaction processing abilities of BFT-based consensus protocols\footnote{Tendermint protocol used by Cosmos network able to process thousands of transactions per second \cite{tendermint}}, let them to scale many sub-blockchains by processing their inter-blockchain transactions.
%In fact, PoW-based sub-blockchains able to process few dozens of transactions per second and presumably only sub-set of their transactions will be inter-blockchain transactions and processed by blockchain connector framework.
%This is very convenient in order to scale to many sub-blockchains, as sub-blockchains are able to process few dozens of transactions according to our evaluations presented in Section \ref{sec:integrationEva}.
%Moreover, presumably only sub-set of transactions in sub-blockchains will be inter-blockchain transactions and send to the blockchain connector framework.


%In parallel to this role, today's blockchain protocols offer simple blockchain client models.
%For example, in case of Bitcoin, nodes can participate in the network as \textit{thin clients}\footnote{\url{en.bitcoin.it/wiki/Thin_Client_Security\#Thin_Clients$}} and send transactions %without block mining or downloading the entire copy of the blockchain. 




SECURITY
8 MARCH DEPRECATED
%The more work a  PoW-based blockchain contains, the more secure it is against threats targeting its integrity, as noted in Section \ref{sec:metrics}.
%Yet in Hybrid-IoT, we propose to divide IoT devices into subgroups and form sub-blockchains.
%Clearly, if total work in each sub-blockchain decreases, it would be easier for a malicious party to generate a longer blockchain and destroy data accountability and integrity.
%By frequent block generation and low stale block generation rates, sub-blockchains may be as robust as the unique blockchain.
%In the following, we quantitatively analyze total work that both unique blockchains contain and sub-blockchains contain, by exploiting the Bitcoin simulator presented in Section \ref{sec:simulatorSettings} for 100 minutes of system execution.


..
..
..
2 li versiyon
\iffalse
%\textbf{Hybrid-IoT.} 
%One of the biggest challenges in the integration of blockchain into IoT ecosystems is scalability.
%In fact, due to the massive number of devices and resource constraints, employing blockchain mechanisms in IoT is particularly challenging.
%The optimal blockchain architecture has to scale to many IoT devices (they become the peers on the blockchain network), and it should be able to process a high throughput of transactions.
%To this end, in this paper we propose a hybrid blockchain architecture, that we call Hybrid-IoT. 
%Hybrid-IoT exploits both PoW-based and BFT-based blockchains.
%First, PoW-based blockchains are used to achieve distributed consensus among many IoT devices as being blockchain peers.
%We define a set of PoW-based blockchain-IoT integration metrics that clarify prerequisites of successful deployment.
%We observed that, by forming multiple PoW-based sub-blockchains that are containing few hundreds of IoT devices that are geographically close to each other, high performance (i.e. high transaction throughputs and low block propagation delays) can be achieved.
%Given that, Hybrid-IoT leverages on a BFT-based multiple blockchain connector framework such as Polkadot\footnote{polkadot.network} and Cosmos\footnote{cosmos.network} in order to achieve interoperability among sub-blockchains.


%\textbf{This work.}
%In this paper, as a first step, we focus on the challenging issue of adapting PoW-based blockchains to the IoT domain by generating sub-blockchains.
%In fact, generating sub-blockchains is not a straightforward task, where both performance and security properties of sub-blockchains have to be considered.
%ELENA: explain what sweet spot setting is
%GOKHAN: Rewritten.
%To this end, we define set of PoW-based blockchain-IoT integration metrics to clarify prerequisites of successful deployment evaluate performance.
%By exploiting the integration metrics we evaluate performance of the integration and by varying block sizes and block generation intervals, device locations, and number of devices as blockchain peers.
%According to our observations, we define a set of rules to regulate sub-blockchain generation without sacrificing security properties, referred to as sweet-spot settings.
%We define the Hybrid-IoT architecture with three roles for IoT devices.
%Moreover, we evaluate the performance of IoT devices with regards to their roles by performing stress test and varying sub-blockchain sizes.
\fi



..
..
..
eski versiyon
\iffalse
%One of the biggest challenges in the integration of blockchain into IoT ecosystems is scalability.
%In fact, due to the massive number of devices and resource constraints, employing blockchain mechanisms in IoT is particularly challenging.
%The optimal blockchain architecture has to scale to many IoT devices (they become the peers on the blockchain network), and it should be able to process a high throughput of transactions.
%To this end, in this paper we propose a hybrid blockchain architecture, that we call Hybrid-IoT. Hybrid-IoT exploits both PoW-based and BFT-based blockchains.
%First, PoW-based blockchains are used to achieve distributed consensus among many IoT devices as being blockchain peers.
%(\textbf{THE PART BELOW I DO NOT UNDERSTAND AND I CANNOT SEE ITS POINT})
%We extensively evaluated performance of the PoW-blockchains in IoT setting in order to assess best practices.
%In that, we observed that blockchains containing few hundreds of IoT devices that are geographically close to each other achieve high performance.
%Given that, Hybrid-IoT includes multiple PoW-blockchains, referred to as sub-blockchains, and a BFT-based multiple blockchain connector framework such as Polkadot\footnote{polkadot.network} and Cosmos\footnote{cosmos.network} in order to achieve interoperability among sub-blockchains.
..
..
..
%\textbf{This work.} In this paper, as a first step, we focus on the challenging issue of adapting PoW-based blockchains to the IoT domain by generating sub-blockchains.
%In fact, generating sub-blockchains is not a straightforward task, where both performance and security properties of sub-blockchains have to be considered.
%As such, we have to achieve high performance with high transaction throughputs and low block propagation delays.
%To this end, we propose a set of rules in generating sub-blockchains to achieve high performance, without sacrificing security properties, referred to as sweet-spot settings.
%(\textbf{PERFORMANCE NEEDS TO BE DEFINED}) 
% GOKHAN: Done.
%By exploiting sub-blockchain approach we design the Hybrid-IoT architecture.
%Moreover, we have defined three roles for IoT devices with regards to their capabilities. 
%(\textbf{SHOULD BE MORE PRECISE BELOW, AKA... WE DO CERTAIN TYPE OF EXPERIMENTS TO EVALUATE AND DESCRIBE THEM BRIEFLY})
%We extensively evaluate performance of generating sub-blockchains by varying block sizes and block generation intervals, device locations, and number of devices as blockchain peers.
%Moreover, 
%and security of generating sub-blockchains, by  
%We extensively evaluate performance and security of generating sub-blockchains, by  
\fi




%Sweet-spot settings:  IoT devices that are geographically close to each other and frequently communicating with each other should be in the same sub-blockchain, sub-blockchains should contain neither too few nor too many IoT devices, key blockchain system parameters, i.e. block size and block generation interval, should be set in such a way that ensures to achieve low stale block generation rates and high decentralization degrees.





ARCHITECTURE


\iffalse
We have to connect sub-blockchains to each other.
To this end, Hybrid-IoT exploits a  BFT-based multiple blockchain connector framework such as Polkadot and Cosmos to perform secure and trust-free inter-blockchain transactions.
We present an example of Hybrid-IoT architecture containing two sub-blockchains in Figure \ref{fig:architecture}.
The main advantage of using BFT-based blockchain as a multiple blockchain connector is achieving high transaction throughputs with low latencies \cite{blockchainSurvey}.
Transaction throughputs of the PoW-based sub-blockchains will be much less than the BFT-based multiple-blockchain connector framework. 
Moreover, presumably only sub-set of transactions in sub-blockchains will be inter-blockchain transactions and send to the connector framework.
As long as connector framework is able to execute and transmit inter-blockchain transactions with very low latency, adding new sub-blockchains generated with the sweet-spot settings do not overwhelm and degrade execution in the Hybrid-IoT. 
Therefore, each new sub-blockchain can preserve its ratio of the transaction throughput to number of devices.
Given that, we claim that, Hybrid-IoT achieves linear scalability in number of devices and transaction throughput of the system.
%\footnote{ripple.com/dev-blog/ripple-consensus-ledger-can-sustain-1000-transactions-per-second}

 \begin{figure*} [h] 
	\centering
	\includegraphics[width=\textwidth]{figures/newArchitecture.png}
	\caption{Hybrid-IoT} \label{fig:architecture}
\end{figure*}
\fi





\iffalse
%In that, in Hybrid-IoT, devices with different capabilities take different roles.
In order to group IoT devices on some common blocks and identify device roles in blockchain systems, we refer to the IoT device classification presented in \cite{ourPaper2}. 
In \cite{ourPaper2}, IoT devices, aka smart objects, have been classified into three groups according to their capabilities, referred to as smartness levels, namely; first, second, and third smartness levels.
At the first smartness level, IoT devices have a very limited capacity by being able only to act as basic sensors, for sensing data from the environment.
Sensors can not process data, whereas they periodically sense the raw data and send it to the cloud or central data processors.
%like Complex Event Processing (CEP) systems.
At the second smartness level, devices have a limited capacity and computing power, making them able only to  perform basic operations by their own (e.g if/else conditions, sum, multiply), such as Arduino Yun.
Whereas, at the third smartness level, devices have enough capacity and computing power for performing more complex operations by their own, such as Raspberry Pi Model B.
\fi


%\textbf{Motivations} : 
%\textbf{Transparency and accountability} As discussed previously, blockchain is replicated among every peer and newly generated blocks are shared to the network. As such, blockchain technology offers great transparency. Recording every transaction ensures accountability, as such blockchain data structure is kind of ledger containing history of every operation performed that are visible to all parties participating (in public blockchains they are publicly visible).  

%We propose to integrate blockchain technology into IoT domain by exploiting its foundational properties to solve some important problems of the IoT domain. 

DECENTRAZLIATION, SECURITY, GLOBAL IDENTIFICATION
By having the potential to solve crucial problems of the IoT domain, foundational properties of the blockchain technology, such as its tamper-proof and decentralized nature and strong security, offers great promises for IoT domain.
Such foundational properties give shape to proposed multi blockchain architecture. 
%Let us discuss how blockchain technology fits to IoT domain by listing beneficial foundational properties of the blockchain technology and how they can help IoT domain in the following as \textit{security, decentralization, transparency} and \textit{identification}.




%Cryptography forms a central part of blockchain protocols. 
%Cryptography is used to protect the integrity of the blockchain, where every block of the blockchain contains a hash of the previous block. 
%Changing contents of a block requires the modification of all following blocks. 
%Additionally, all popular blockchains use \textit{Digital signature algorithms} to cryptographically sign transactions sent among peers, specifically the Elliptic Curve Digital Signature Algorithm (ECDSA) is used to authenticate transactions. 

%\textbf{Security}
%Since blockchain technology uses cryptography for data and transaction encryption, even  every peer of the network has all blockchain data and able to compute everything, the underlying meaning of the information is completely obfuscated from original data\footnote{blog.ethereum.org/2016/01/15/privacy-on-the-blockchain/}.
%Considering security issues that we are facing today in IoT domain, such as unsecured communication among devices and poor authentication of IoT devices, foundational properties of blockchain technology may improve integrity and authenticity of the IoT applications. 
%In Section \ref{sec:security} we analyze and test security properties of proposed architecture.  



%\textbf{Decentralization} 
%Blockchain technology is a peer to peer decentralized technology, without a centralized intermediary. 
%Peers of the network agree on the state of the blockchain by achieving consensus, which overcomes the problem of a single point of failure. 
%Indeed, assuming majority of the peers of the network are active and honest, blockchain ensures that even if some peers drop out temporarily from the network, consensus among honest peers will be achieved. 
%Considering today's IoT, where IoT is evolving into a loosely coupled, decentralized system of cooperating smart objects, we have to consider the IoT domain as independent objects with the ability to cooperate without knowing or trusting each other. The decentralized nature of blockchain technology is a great fit for today's smart objects. 



\textbf{Resource restricted IoT Devices} 
IoT devices show great diversity regarding their capabilities \cite{Nistir, ourPaper2,ituStandard}. 
Devices with low processing capabilities and storage space will be cumbersome for integration of blockchain technology into IoT domain. 
As we discuss in \ref{sec:architecture}, we propose to use multiple blockchains to decrease resource usage of blockchain protocols. 
Additionally, we propose the use of light blockchain protocols to increase collaboration of resource restricted devices in blockchain systems, where we showed performance results in Section \label{sec:lightPerformance}.

%\textbf{Ever changing needs of IoT domain}
%IoT technology is expanding and changing very fast, therefore new uses emerges according to that. Previously discussed smart contract concept with increased programming capabilities of blockchains, e.g. Ethereum, offers great promises to overcome such challenges. Indeed, we propose to use of smart contract concept of blockchain technology in order to perform complex use cases with proposed architecture.
%\textbf{Protection and security of devices}
%IoT devices with poor authentication and authorization mechanisms generates important vulnerabilities to any system. In Section \ref{sec:security} we discuss security threats to proposed architecture in detail, how they may effect the system and how to protect system against such threats.
%\textbf{Limited monitoring and lack of standards on IoT devices} Today, many IoT Systems are poorly designed and implemented with different protocols and technologies\footnote{www.iot.ieee.org/newsletter/january-2017/iot-and-blockchain-convergence-benefits-and-challenges.html}. Additionally, there is limited guidance for life cycle management of IoT device and lack of standards. Therefore, we propose a flexible blockchain architecture, where blockchain protocols 





\iffalse
%d


%Massive number of IoT devices, expected to be around twenty billions, according to ITU \cite{ituIoT}, is an important issue that gives rise to serious concerns for the future of the domain. 
%Additionally, Device and data security, data accountability and device identification of IoT systems always in question and mostly very fragile and weak. 
%Indeed, considering growth of the IoT market and newly interconnected devices increase attack surface simply because each of them can become the weakest link and exploited \cite{learningIoTsecurity}. 


\subsection{Evaluation \rom{4}: Cost of the Proof of Work Consensus}\label{sec:eva4}
In order to solve the PoW puzzle, miner devices have to use their resources (e.g. in case of Bitcoin CPU/GPU) and use electricity.
In what follows, we discuss cost of the PoW consensus algorithm, on an example case of Bitcoin by exploiting the Bitcoin simulator presented in Section \ref{sec:simulatorSettings}. 
Bitcoin miners perform double SHA-256 functions to take hash of the string representing transactions and a nonce \cite{bitcoinEnergy}. 
Hashing operation is repeated by varying the nonce value until a hash result less then the pre-defined target value has been found.
In Bitcoin blockchain, difficulty is used to regulate target value according to total hash power in the Bitcoin network to have 10 minutes average block generation interval.
With total hash rate of $HR$ and difficulty $Diff$, the formula\footnote{en.bitcoin.it/wiki/Difficulty} to calculate the expected time to find a new block $T_{E}$ is:

\begin{align}
T_{E} \approx \frac{Diff * {2^{32}}}{HR}    
\end{align}


Based on this formula, we evaluate the cost, difficulty and hash rate relation of Bitcoin's PoW algorithm on IoT domain. 
We have used Raspberry Pi Model B \footnote{www.raspberrypi.org/products/raspberry-pi-1-model-b/} as a reference IoT device to calculate it's electricity consumption cost. 
Single Raspberry Pi Model B has 0.2 mega hash per second (0.2 MH/s) and uses 3.5 watts of electricity per hour (3.5 W/h)\footnote{$en.bitcoin.it/wiki/Non specialized_hardware_comparison$}.
We picked the Netherlands as a reference country in calculating electricity costs.
In the Netherlands electricity cost is around 0.20\$ for kilo watts per hour(KW/h)\footnote{$ec.europa.eu/eurostat/statistics-explained/index.php/Electricity_price_statistics$} for household usage.
Let us first present the relation of number of devices to total hash power and electricity cost on system execution for one day in Figure \ref{fig:cost1}.
Total hash power in the system and electricity consumption costs of IoT devices change in direct proportion to number of devices in the system.


\begin{figure} [H]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/deviceHashCost.png}
	\caption{Cost - difficulty relation \label{fig:cost1}}
\end{figure}


Secondly, we evaluate the relation of cost, block generation interval and network latency (nodes' location) to generate 10000 blocks with 500 KB size.  
To this end, we refer to experiment results presented in Evaluation \rom{2}, that demonstrates number of blocks generated in 100 minutes of system execution in different location settings (the Netherlands, Europe, World).
We present cost analysis results in Table \ref{tab:costAnalysis}.

\begin{table}  
\centering
\begin{tabular} {|c|cc|cc|cc|} %{ |l *{6}{D{.}{.}{4}}} {|ccc|cc|cc|}
\toprule
\textbf{Interval:} & \multicolumn{2}{c}{\textbf{Netherlands}} & \multicolumn{2}{c}{\textbf{Europe}} & \multicolumn{2}{c}{\textbf{World}} \\
\cmidrule(lr){2-3}  
\cmidrule(lr){4-5} 
\cmidrule(lr){6-7} 
\textbf{Results/} & \multicolumn{1}{c}{$Cost$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Cost$} & \multicolumn{1}{c}{$Stale$} & \multicolumn{1}{c}{$Cost$} & \multicolumn{1}{c}{$Stale$}  \\
\textbf{Cases}	  & \multicolumn{1}{c}{$(\$)$} & \multicolumn{1}{c}{$Rate$}  & \multicolumn{1}{c}{$(\$)$} & \multicolumn{1}{c}{$Rate$} & \multicolumn{1}{c}{$(\$)$} & \multicolumn{1}{c}{$Rate$}\\
\midrule
\textbf{10 minutes}   & 1.81 					& 0\%        					&  1.81  						&0\% 						& 1.97						&  0\%\\ 
\hline
\textbf{5 minutes}   &  1.32					& 0\%        					&  1.32  						&0\% 						& 1.40						&  0\%\\ 
\hline
\textbf{1 minute}   &  0.21						& 1.76\%        				&  0.24							&5.14\% 					& 0.24						&  8.22\%\\  
\hline
\textbf{30 seconds}   &  0.13					& 5.15\%        				&  0.13							&  12.87\% 					& 0.14						& 14.11\%\\ 
\hline
\textbf{10 seconds}   &  0.09					& 32.49\%        			    &  0.10 						&  33.31\% 					& 0.12						&  41.34\%\\ 
\hline
\textbf{5 seconds}   &  0.14					& 47.66\%        				&  0.15							&  51.80\% 					& 0.16						&  53.12\%\\ 
\bottomrule             
\end{tabular}
\caption{Cost analysis} \label{tab:costAnalysis} 
\end{table}


First important aspect to examine is the total cost.
We have observed that, with shorter block generation intervals total costs are less as devices have to operate less amount of time to produce 1000 blocks.
However, in 5 seconds setting due to very high stale block rate, total cost is higher than 10 seconds and 30 seconds setting.
In evaluating total cost of the system, another important aspect to consider besides total cost of the energy waste. 
Energy spent to generate and propagate a stale block have to be considered as a waste of energy, as stale blocks do not included to blockchain. 
Shorter block generation intervals imply higher stale block generation rates, and thus higher waste of energy.
For example, in 5 seconds block generation interval setting, stale block generation rates for all location settings are around 50\%.
This signifies that around half of the consumed electricity and thus total cost is unutilized.
Thus, such systems are very inefficient, and they do not comply with the efficiency metric. 
As discussed in Evaluation \rom{2}, the Netherlands setting shows the lowest stale block generation rates and thus the most efficient and cheapest setting. 
Given all, we conclude that, short block generation intervals in low network latency settings with low stale rates should be used for maximum energy efficiency and low electricity costs.











%d
\subsection{Evaluation \rom{5}: Blockchain types}\label{sec:eva5}
Today, different types of blockchains are in use to address requirements of different businesses and domains.
Blockchains are mostly categorized into three groups as; \textit{public, private} and \textit{consortium} blockchains.
Public blockchains referred as permissionless blockchains, whereas private and consortium blockchains are referred as permissioned blockchains.
Blockchains in different groups show great difference in terms of their methodology to achieve consensus and rights assigned to the blockchain nodes.
In the following, we evaluate different types of blockchains regarding whether they are suitable for IoT domain or not.


\subsubsection{Public blockchains}\label{sec:publicBlc}
In public blockchains,any device with an active internet connection can send transactions, read the blockchain, and take part in the consensus process.
Public blockchains do not depend on central authority or trusted entity, and they are close to be fully decentralized. 
As long as majority of the mining power in the network is acting honestly, malicious parties can not divert the blockchain.
However, IoT devices have limited resources and thus limited mining powers, and this is a problem in designing public blockchain.
In example case of Bitcoin, Raspberry Pi, has 0.2 MH/s mining power\footnote{$en.bitcoin.it/wiki/Non specialized_hardware_comparison$}, whereas a specialized mining device AntMiner S9 \footnote{www.amazon.com/Bitmain-Antminer-S9-Bitcoin-Efficiency/dp/B075MH4HSL} has 14 GH/s mining power.
That means, even a single specialized mining hardware con oppress millions of standard IoT devices, and may forge system to operate maliciously. 
Given that, public blockchain is not suitable for IoT domain.


\subsubsection{Private blockchains}\label{sec:privateBlc}
In private blockchains, right of writing to the blockchain and participating in the consensus process is only kept to one entity, whereas read access may be public or may be given to some entities with limited context. 
As consensus process is handled by one trusted source, malicious parties with specialized hardwares can not divert blockchain actions like as in public blockchains.
To divert a private PoW blockchain, attacker has to both gain access to miner devices and have the majority of the hashrate. % to ensure its blocks are generated faster than the rest of the network combined.
Private blockchains offer much faster block generation and confirmation times, as device faults can be corrected manually and devices are supposed to be very well connected. 
Furthermore, the entity that is running private blockchain can change blockchain rules easily and divert malicious activities.
However, this will cause big problems against cooperation of different parties as only one party is in charge of consensus and others have to trust the authority.
Indeed, private blockchains are centralized and they lack trustless communication and cooperation of different parties which is one of the biggest advantages of using blockchain technology.
Given all, we conclude that, private blockchains offer some advantages and thus can be suitable for some IoT use-cases, however they lack some important features of public blockchains like decentralization.


\subsubsection{Consortium blockchains}\label{sec:consortiumBlc}
In consortium blockchains, writing to the blockchain and taking part in the consensus process is distributed into set of nodes, whereas read access may be given to some entities with limited context or it may be public.  
Subset of nodes from different parties can be authorized to write to the blockchain and take part in consensus process.
By doing so, all parties take part in the consensus process, and as long as majority of the mare honest,they can protect the integrity of the blockchain from dishonest parties.
Similar with private blockchains, attacker both needs to gain access to pre-selected authorized nodes on consensus and have the majority of the mining power to maliciously alter the blockchain.
In contrast to private blockchains, partial decentralization in consortium blockchains allow cooperation of different parties. 
In consortium blockchains, sybil resistance to off-chain can be increased by holding mining power in trusted resources.
Ideally, all parties should contribute to consensus process with equal mining power to achieve decentralization and communicate without trust. 
Even though consortium blockchains does not provide fully decentralized consensus, they allow cooperation of different parties with less security threats from malicious parties.   
Given all, we conclude that, consortium blockchains can be a suitable solution in designing an IoT application containing various parties as services providers or device vendors.
%The way people try to use PoW for consortium networks does not cause excess power usage: low difficulty, low powered device/s.








%d
\subsection{Evaluation \rom{6}: IoT devices as blockchain nodes}\label{sec:eva6}
In IoT domain, device capabilities are extremely heterogeneous.
To group IoT devices on some common blocks, we refer to the device classification based on their capabilities as presented in \cite{ourPaper2}.
In \cite{ourPaper2}, smartness of the IoT devices, aka smart objects, have been classified into three smartness levels as; first, second, and third smartness levels.
In the following, we examine how IoT devices that are classified into different smartness levels can be part of the blockchain. 


\subsubsection{First smartness level -- Sensors}\label{sec:firstLevelDevice} 
At the first level, devices have a very limited capacity, being able only to act as  basic sensors, for sensing data from the environment.   
Sensors can not process data, whereas they periodically sense the raw data and send it to the cloud or central data processors like Complex Event Processing (CEP) systems.
Thus, such devices can not be peers in the blockchain network. 
The ideal way to somehow connect those devices to the blockchain network is connecting them to other devices that are peers of the blockchain network. 
If we consider many sensors that are continuously sensing raw data, storing all raw data in the blockchain will be a big hurdle against scalability of the blockchain system.
Therefore, raw data sent by sensors should be processed by higher capability devices or data processing systems that are peers of the blockchain network.
Sensor data needs to be stored in the cloud or servers.
Peers, however, may form transactions and send it to the blockchain network after data processing, if required.
Given all, devices with first smartness level can not directly participate in blockchains, but they can connect to smarter intermediary device indirectly participate.

\subsubsection{Second smartness level -- Devices with low capabilities}\label{sec:secondLevelDevice} 
At the second level, devices have a limited capacity and computing power, making them able only to  perform basic operations by their own (e.g if/else conditions, sum, multiply).
For example, Arduino Yun\footnote{store.arduino.cc/arduino-yun} can be categorized as a device with second level smartness.
Those devices are able to run basic operating systems such as Alpine Linux\footnote{alpinelinux.org}, and they can connect to the blockchain network.
As such devices run am operating systems and able to process data, they can participate in the blockchain network by performing some simple tasks, like sending transactions.
In parallel with that, today's blockchain protocols offer simple client models.
For example, in case of Bitcoin, nodes can participate in the network as \textit{thin clients}\footnote{$en.bitcoin.it/wiki/Thin_Client_Security\#Thin_Clients$}.
Thin clients perform simpler operations like sending transactions and thus require less resources. 
As such, thin clients do not download all blockchain but they download a complete copy of the headers for all blocks in the entire blockchain and they do not participate in the consensus process.
Given all, devices with second smartness level can take simple client roles that do not require to mine blocks are participate in consensus process, like thin client role in case of Bitcoin. 


\subsubsection{Third smartness level -- Devices with high capabilities}\label{sec:thirdLevelDevice} 
At the third level, devices have enough capacity and computing power for performing more complex operations by their own.
For example, Raspberry Pi Model B\footnote{raspberrypi.org/products/raspberry-pi-1-model-b} can be categorized as a device with third level smartness.
Those devices run more advanced operating systems like Raspbian\footnote{www.raspbian.org}, and they are able to connect and participate in the blockchain network. 
Such devices can perform more complex blockchain tasks than devices with lower smartness level, such as mining blocks and taking part in the consensus process. 
However, their capabilities are not enough to solve very complex PoW puzzles to mine a block, or propagate big blocks.
For example, in case of Bitcoin, Raspberry Pi Model B has 0.2 mega hash per second (0.2 MH/s) and with the difficulty setting in Bitcoin network in late 2017, it would take more than 1000 years to solve the PoW puzzle for a million Raspberry Pi Bs.
Moreover, their bandwidth capabilities are limited, therefore very big block sizes or very short block generation interval settings are not suitable for such devices (as discussed in Evaluation \rom{1}).
Given all, devices with the third level of smartness can participate in the blockchain networks as full peers, by carefully setting consensus parameters and blockchain rules such as block size and block generation interval.

\fi


















%Since inter-chain transactions affect current status of both of the blockchains, and to preserve integrity and accountability, inter-chain transactions will be recorded by multiple blockchain connector framework, presumably in its local blockchain (as its done in Polkadot\cite{polkadot}). As such, overall system traceability and consensus will be ensured.
\iffalse
\textbf{Multichain connector framework: }
\textbf{polakdot.}
Polkadot \cite{polkadot}. presents a vision for heterogeneous multi-chain framework. 
In this framework, rather than presenting a single chain, Polkadot provides the bedrock \textit{relay-chain} upon which a large number of blockchains may be hosted (called as \textit{parachains}). In Polkadot, relay chain will have its own security and security will be shared across the parachains(blockchains that are connected to the Polkadot framework). Polkadot provides trust-free transactions between independent parachains. Polkadot framework provides trust free bridges allowing transactions to be routed from a parachain to another. Polkadot parachains communicates via interchain communication, so they have some sort of communication channel between them. 

Polkadot network consists four basic roles to keep up the network, namely \textit{Validator}, \textit{Nominator}, \textit{Collator} and \textit{Fisherman}.
Validator helps seal new block on the Polkadot network, which refers to relay chain and all parachains. 
A Validator must run a relay-chain implementation with high availability and bandwidth, in order to be ready to accept new block on a nominated parachain. 
Validator receives the block from nominated parachain, validates it, and then republishes the block. 
%Validation of a block requires fully-synchronized database of the parachain, but since maintaining all of the parachains is not reasonable, validator will nominate the task of devising a suggested new parachain block to collator. 
Firstly, validator subgroups validates all new parachain blocks, then validators must ratify the relay-chain block itself
. 
A validator is punished if it does not act honestly or does not fulfill its duty to find consensus.  
Nominator is a stake-holding party contributing security bond of a validator. 
Nominators select validators that they trust to act responsibly in maintenance of the network, and they place risk capital to such validator. 
%They receive increase or decrease in their deposit according to the bond's growth.
Collator assists validator in producing valid parachain blocks. 
Collators maintain a "full-node" in particular parachain, meaning that they can retain all information required to author new blocks and execute transactions. Collator executes transactions to create unsealed block and provides the block to the validators with zero-knowledge proof.    
Fishermen is not an active part and does not take role in block authoring process. Fishermen, are independent "bounty-hunters", they get their reward by proving one bonded party acted illegally.

Polkadot achieves low-level consensus over a set of mutually agreed and valid block through asynchronous \textit{Byzantine Fault Tolerant (BFT)} algorithm. 
Polkadot determines set of validators and incentives validators by utilizing \textit{Proof of Stake (PoS)} based selection criteria. 
In Polkadot, parachains' header are sealed within the relay-chain block ensuring no reorganisation or "double-spending" is possible after confirmation of block. 
Additionally, Polkadot also provides strong guaranty that the state transitions of parachains are valid.  Polkadot parachains communicates via interchain communication, so they have some sort of communication channel between them.


Cosmos [10] is a proposed multi-chain system in the
same vein as side-chains, it describes multiple chains (operating in
zones) each using individual instances of Tendermint, together
with a means for trust-free communication via a
master hub chain.
This interchain communication is limited
to the transfer of digital assets ( about tokens")
rather than arbitrary information, however such interchain
communication does have a return path for data,
e.g. to report to the sender on the status of the transfer.
Validator sets for the zoned chains, and in particular
the means of incentivising them, are, like side-chains, left
as an unsolved problem. The general assumption is that
each zoned chain will itself hold a token of value whose in-

ation is used to pay for validators. Still in the early stages
of design, at present the proposal lacks comprehensive details
over the economic means of achieving the scalable
certainty over global validity. However, the loose coherence
required between the zones and the hub will allow
for additional 
exibility over the parameters of the zoned
chains compared to that of a system enforcing stronger
coherence.
\fi






































LOCATION EXPERIMENTS
\iffalse
%Netherlands
\begin{table} 
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  }        & {\bf Total }  		&  \textbf{Stale} 		& \textbf{Genuine} 		 &{\bf Stale}   	&{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Gen.}           &\textbf{Blocks}		& \textbf{Blocks} 		& \textbf{Blocks}   	&\textbf{Rate} 		&\textbf{Prop.}   &\textbf{Traffic} & {\bf (TX/s)}\\ 
         \textbf{Intrvl(s)}      & 			  			&	 			    	&                   	&              		&\textbf{Delay(s)}&\textbf{(Kbps)} & \\
     	\hline
         \textbf{10 minutes} 	 & {\bf 9.65}           & \textbf{0.00} 	     &{\bf 9.65} 			  &  {\bf 0.0\%}	 & {\bf 7.13}   & {\bf 13.37}    & {\bf 3.21 TX/s}  \\
        \hline
         \textbf{5 minutes}		 & {\bf 18.65}          & \textbf{0.00} 		 &{\bf 18.65}  			  &  {\bf 0.0\%} 	 & {\bf 6.89}   & {\bf 26.74}    & {\bf 6.21 TX/s}  \\
        \hline
         \textbf{1 minutes}		 & {\bf 92.14}          & \textbf{0.66} 	     &{\bf 91.48}     		  &  {\bf 0.71\%} 	 & {\bf 9.11}   & {\bf 136.45}      & {\bf 30.71 TX/s} \\
        \hline
         \textbf{30 seconds} 	 & {\bf 165.20}         & \textbf{2.59} 	     &{\bf 162.61}            &  {\bf 1.56\%}    & {\bf 20.45}   & {\bf 499.78}      & {\bf 54.2 TX/s}\\
        \hline
         \textbf{10 seconds}     & {\bf 346.58}         & \textbf{101.39} 	     &{\bf 245.19}            &  {\bf 29.25\%}   & {\bf 314.08}   & {\bf 14762.93}     & {\bf 81.73 TX/s} \\
        \hline 
         \textbf{5 seconds} 	 & {\bf 350.68}         & \textbf{161.18} 	     &{\bf 189.50}            &  {\bf 45.96\%}   & {\bf 815.39}  & {\bf 41378.1}     & {\bf 63.16 TX/s} \\
        \hline       
    \end{tabular}
\caption{Evaluation \rom{1} Netherlands cities setting} \label{tab:eva2Netherlands}
\end{table}

%Europe
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  }        & {\bf Total }  		&  \textbf{Stale} 		& \textbf{Genuine} 		 &{\bf Stale}   	&{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Gen.}           &\textbf{Blocks}		& \textbf{Blocks} 		& \textbf{Blocks}   	&\textbf{Rate} 		&\textbf{Prop.}   &\textbf{Traffic} & {\bf (TX/s)}\\ 
         \textbf{Intrvl(s)}      & 			  			&	 			    	&                   	&              		&\textbf{Delay(s)}&\textbf{(Kbps)} & \\
     	\hline
         \textbf{10 minutes} 	 & {\bf 9.96} 			& \textbf{0} 		     &{\bf 9.96}  			  &  {\bf 0\%}	     & {\bf 16.69s}     & {\bf 13.54}  &{\bf 3.32 TX/s}\\
        \hline
         \textbf{5 minutes}		 & {\bf 16.39}		    & \textbf{0}		     &{\bf 16.39}  			  &  {\bf 0\%} 		 & {\bf 13.62s}     & {\bf 27.92}  &{\bf 5.46 TX/s}\\
        \hline
         \textbf{1 minutes}		 & {\bf 93.6} 			& \textbf{4.82} 		 &{\bf 88.78}     		  &  {\bf 5.14\%} 	 & {\bf 14.32s}     & {\bf 140.06}  &{\bf 29.59 TX/s}\\
        \hline
         \textbf{30 seconds} 	 & {\bf 170.54}         & \textbf{21.94} 	     &{\bf 148.6}             &  {\bf 12.87\%}   & {\bf 38.55s}     & {\bf 527.75}  &{\bf 49.53 TX/s}\\
        \hline
         \textbf{10 seconds}     & {\bf 314.04}         &\textbf{104.60} 	     &{\bf 209.44}            & {\bf 33.31\%}    & {\bf 355.99s}    & {\bf 15237.3} &{\bf 69.81 TX/s}\\
        \hline 
         \textbf{5 seconds} 	 & {\bf 301.25}         &\textbf{156.04}         &{\bf 145.21}            & {\bf 51.80\%}    & {\bf 918.98s}    & {\bf 43931.4} &{\bf 37.83 TX/s}\\
        \hline       
    \end{tabular}
\caption{Europe cities setting} \label{tab:eva2Europe}
\end{table}

%World
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  }        & {\bf Total }  		&  \textbf{Stale} 		& \textbf{Genuine} 		 &{\bf Stale}   	&{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Gen.}           &\textbf{Blocks}		& \textbf{Blocks} 		& \textbf{Blocks}   	&\textbf{Rate} 		&\textbf{Prop.}   &\textbf{Traffic} & {\bf (TX/s)}\\ 
         \textbf{Intrvl(s)}      & 			  			&	 			    	&                   	&              		&\textbf{Delay(s)}&\textbf{(Kbps)} & \\
     	\hline
         \textbf{10 minutes} 	 & {\bf 9.96} 			& \textbf{0} 		     &{\bf 10.96}  			  &  {\bf 0\%}	     & {\bf 20.03s}    & {\bf 13.64}	 &{\bf 3.32 TX/s}\\
        \hline
         \textbf{5 minutes}		 & {\bf 15.45}		    & \textbf{0}		     &{\bf 15.45}  			  &  {\bf 0\%} 	     & {\bf 17.73s}    & {\bf 27.46}     &{\bf 5.15 TX/s}\\
        \hline
         \textbf{1 minutes}		 & {\bf 96.52} 		    & \textbf{7.93} 		 &{\bf 88.59}     		  &  {\bf 8.22\%} 	 & {\bf 20.85s}    & {\bf 140.78}    &{\bf 29.53 TX/s}\\
        \hline
         \textbf{30 seconds} 	 & {\bf 169.46}         & \textbf{23.91} 	     &{\bf 145.55}            &  {\bf 14.11\%}   & {\bf 52.1s}     & {\bf 592.76}    &{\bf 48.51 TX/s}\\
        \hline
         \textbf{10 seconds}     & {\bf 331}            &\textbf{136.83} 	     &{\bf 194.17}            &  {\bf 41.34\%}   & {\bf 392.74s}   & {\bf 16777.5}   &{\bf 64.72 TX/s}\\
        \hline 
         \textbf{5 seconds} 	 & {\bf 303.28}         &\textbf{161.1}         &{\bf 142.18}             &  {\bf 53.12\%}   & {\bf 1000.49s}   & {\bf 45021.32} &{\bf 47.39 TX/s}\\
        \hline        
    \end{tabular}
\caption{World cities setting} \label{tab:eva2World}
\end{table}

\fi











time - size experiments

  
\iffalse
\begin{table}
    \centering
    \scriptsize
    \begin{tabular} {*{8}{c}} %{|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 10.82} 			& \textbf{0.00} 		 &{\bf 10.82}  			  &  {\bf 0.00\%}	 & {\bf 156.77}  &{\bf 276.50}  & {\bf 72.13}  \\
         
         
        \hline
         \textbf{5 MB}		 & {\bf 10.27}		    & \textbf{0.00}		     &{\bf 10.27}  			  &  {\bf 0.00\%} 	 & {\bf 78.35}   &{\bf 134.08} & {\bf 34.23}  \\
        \hline
         \textbf{1 MB}		 & {\bf 12.33} 			& \textbf{0.00} 		 &{\bf 12.33}     		  &  {\bf 0.00\%} 	 & {\bf 14.32}   &{\bf 26.64} & {\bf 8.22} \\
        \hline
         \textbf{500 KB} 	 & {\bf 9.65}           & \textbf{0.00} 	     &{\bf 9.65}              &  {\bf 0.00\%}    & {\bf 7.13}    &{\bf 13.37}  & {\bf 3.21}\\
        \hline
         \textbf{100 KB}     & {\bf 9.33}           & \textbf{0.00} 	     &{\bf 9.33}              &  {\bf 0.00\%}    & {\bf 1.48}    &{\bf 2.74} & {\bf 0.62} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 11.00}          & \textbf{0.00}          &{\bf 11.00}             &  {\bf 0.00\%}    & {\bf 0.72}    &{\bf 1.41} & {\bf 0.36} \\
        \hline      
         \textbf{10 KB}      & {\bf 10.33}          & \textbf{0.00}          &{\bf 10.33}             &  {\bf 0.00\%}    & {\bf 0.17}    &{\bf 0.34} & {\bf 0.06}  \\
        \hline    
    \end{tabular}
\caption{10 minutes block generation interval setting} \label{tab:10min}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 18.84} 			& \textbf{0.91} 		 &{\bf 17.93}  			  &  {\bf 4.83\%}	 & {\bf 201.01} 	 &{\bf 723.40}  & {\bf 119.53}  \\
        \hline
         \textbf{5 MB}		 & {\bf 19.97}		    & \textbf{0.66}		     &{\bf 19.31}  			  &  {\bf 3.30\%} 	 & {\bf 91.73}      &{\bf 288.10}  & {\bf 64.36}  \\
        \hline
         \textbf{1 MB}		 & {\bf 22.33} 			& \textbf{0.00} 		 &{\bf 22.33}     		  &  {\bf 0.00\%} 	 & {\bf 15.44}    	 &{\bf 53.28}   & {\bf 14.88} \\
        \hline
         \textbf{500 KB} 	 & {\bf 18.65}          & \textbf{0.00} 		 &{\bf 18.65}     		  &  {\bf 0.00\%}    & {\bf 6.89}       &{\bf 26.74}   & {\bf 6.21}\\
        \hline
         \textbf{100 KB}     & {\bf 23.00}          & \textbf{0.00} 		 &{\bf 23.00}     		  &  {\bf 0.00\%}    & {\bf 1.46}       &{\bf 5.48}    & {\bf 1.53} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 18.66}          & \textbf{0.00} 		 &{\bf 18.66}     		  &  {\bf 0.00\%}    & {\bf 0.74}       &{\bf 2.82}   & {\bf 0.62} \\
        \hline      
         \textbf{10 KB}      & {\bf 21.66}          & \textbf{0.00} 		 &{\bf 21.66}     		  &  {\bf 0.00\%}    & {\bf 0.17}       &{\bf 0.69}   & {\bf 0.14}  \\
        \hline    
    \end{tabular}
\caption{5 minutes block generation interval setting} \label{tab:5min}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 45.65} 			& \textbf{16.02} 		 &{\bf 26.93}  			  &  {\bf 35.07\%}	 & {\bf 618.57}   	 &{\bf 21215.86}    & {\bf 197.53}  \\
        \hline
         \textbf{5 MB}		 & {\bf 67.30}		    & \textbf{12.11}		 &{\bf 55.19}  			  &  {\bf 17.99\%} 	 & {\bf 214.97}     &{\bf 8718.29}   & {\bf 183.96}  \\
        \hline
         \textbf{1 MB}		 & {\bf 92.47} 			& \textbf{0.66} 		 &{\bf 91.81}     		  &  {\bf 0.71\%} 	 & {\bf 31.95}    	 &{\bf 438.86} & {\bf 61.20} \\
        \hline
         \textbf{500 KB} 	 & {\bf 92.14}          & \textbf{0.66} 	     &{\bf 91.48}             &  {\bf 0.71\%}    & {\bf 9.11}       &{\bf 136.45}  & {\bf 30.71}\\
        \hline
         \textbf{100 KB}     & {\bf 99.00}           &\textbf{0.00} 	     &{\bf 99.00}             &  {\bf 0.00\%}    & {\bf 1.47}       &{\bf 27.40}   & {\bf 6.6} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 96.33}           &\textbf{0.00} 	     &{\bf 96.33}             &  {\bf 0.00\%}    & {\bf 0.76}       &{\bf 14.12}   & {\bf 3.21} \\
        \hline      
         \textbf{10 KB}      & {\bf 101.00}          &\textbf{0.00} 	     &{\bf 101.00}            &  {\bf 0.00\%}    & {\bf 0.17}      &{\bf 3.49}    & {\bf 0.67}  \\
        \hline    
    \end{tabular}
\caption{1 minute block generation interval setting} \label{tab:1min}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 51.28} 			& \textbf{26.67} 		 &{\bf 24.61}  			  &  {\bf 47.99\%}	 & {\bf 1154.07}   &{\bf 49520.10}  & {\bf 164.06}  \\
        \hline
         \textbf{5 MB}		 & {\bf 73.49}		    & \textbf{26.84}		 &{\bf 46.65}  			  &  {\bf 36.52\%} 	 & {\bf 657.17}   	 &{\bf 28528.53}  & {\bf 155.5}  \\
        \hline
         \textbf{1 MB}		 & {\bf 165.91}			& \textbf{8.56} 		 &{\bf 157.35}     		  &  {\bf 5.15\%} 	 & {\bf 52.26}   	 &{\bf 3243.78}  & {\bf 104.9} \\
        \hline
         \textbf{500 KB} 	 & {\bf 165.20}         & \textbf{2.59} 	     &{\bf 162.61}            &  {\bf 1.56\%}    & {\bf 20.45}      &{\bf 639.78} & {\bf 54.2}\\
        \hline
         \textbf{100 KB}     & {\bf 186.41}         &\textbf{0.66} 	         &{\bf 185.75}            &  {\bf 0.35\%}    & {\bf 1.49}       &{\bf 54.85}   & {\bf 12.38} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 187.00}         &\textbf{0.66}           &{\bf 186.34}            &  {\bf 0.35\%}    & {\bf 0.75}       &{\bf 28.24}   & {\bf 6.21} \\
        \hline      
         \textbf{10 KB}      & {\bf 193.33}         &\textbf{0.0}            &{\bf 193.33}            &  {\bf 0.00\%}   & {\bf 0.17}        &{\bf 6.99}   & {\bf 1.28}  \\
        \hline    
    \end{tabular}
\caption{30 seconds block generation interval setting} \label{tab:30sec}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 57.77} 			& \textbf{41.24} 		 &{\bf 16.53}  			  &  {\bf 71.38\%}	 & {\bf 1732.54} &{\bf 151046.00}  & {\bf 110.2}  \\
        \hline
         \textbf{5 MB}		 & {\bf 84.09}		    & \textbf{56.5}		     &{\bf 27.59}  			  &  {\bf 67.18\%} 	 & {\bf 1486.55} &{\bf 100255.03}   & {\bf 91.96}  \\
        \hline
         \textbf{1 MB}		 & {\bf 219.69}         & \textbf{94.18} 		 &{\bf 125.51}     		  &  {\bf 42.86\%} 	 & {\bf 693.22}  &{\bf 30259.26}   & {\bf 83.67} \\
        \hline
         \textbf{500 KB} 	 & {\bf 346.58}         & \textbf{101.39} 	     &{\bf 245.19}            &  {\bf 29.25\%}   & {\bf 314.08}  &{\bf 14762.93}  & {\bf 81.73}\\
        \hline
         \textbf{100 KB}     & {\bf 537.31}         & \textbf{6.21} 	     &{\bf 531.1}             &  {\bf 1.15\%}    & {\bf 5.50}     &{\bf 447.74} &{\bf 35.4} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 562.00}         & \textbf{4.66}          &{\bf 557.33}            &  {\bf 0.82\%}    & {\bf 0.77}    &{\bf 84.55}  & {\bf 18.57} \\
        \hline      
         \textbf{10 KB}      & {\bf 598.66}         & \textbf{0.00}          &{\bf 598.66}            &  {\bf 0.00\%}    & {\bf 0.17}    &{\bf 20.94}   & {\bf 3.99}  \\
        \hline    
    \end{tabular}
\caption{10 seconds block generation interval setting} \label{tab:10sec}
\end{table}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}       &{\bf Average }   & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{prop.}   &\textbf{Traffic} & {\bf (TX/s)} \\ 
        				  & 			  &	 			    &                  &             &\textbf{Delay(s)}&\textbf{(Kbps)}  & \\
        \hline
         \textbf{10 MB} 	 & {\bf 64.26} 			& \textbf{48.20} 		 &{\bf 16.06}  			  &  {\bf 75.00\%}	 & {\bf 1988.84}  &{\bf 273777.66}  & {\bf 107.06}  \\
        \hline
         \textbf{5 MB}		 & {\bf 91.42}		    & \textbf{68.49}		 &{\bf 22.93}  			  &  {\bf 74.91\%} 	 & {\bf 1738.58}  &{\bf 190671.00}  & {\bf 76.43}  \\
        \hline
         \textbf{1 MB}		 & {\bf 232.52} 		& \textbf{128.7} 		 &{\bf 103.87}     		  &  {\bf 55.37\%} 	 & {\bf 1105.55}  &{\bf 69059.33}  & {\bf 69.24} \\
        \hline
         \textbf{500 KB} 	 & {\bf 350.68}         & \textbf{161.18} 	     &{\bf 189.50}            &  {\bf 45.96\%}   & {\bf 815.39}   &{\bf 41378.10}   & {\bf 63.16}\\
        \hline
         \textbf{100 KB}     & {\bf 954.55}         &\textbf{124.51} 	     &{\bf 830.04}            &  {\bf 13.04\%}   & {\bf 57.48}    &{\bf 7249.57}   & {\bf 55.33} \\
        \hline 
         \textbf{50 KB} 	 & {\bf 1120.39}        &\textbf{9.79}           &{\bf 1110.60}           &  {\bf 0.87\%}    & {\bf 4.25}     &{\bf 931.01} & {\bf 37.02} \\
        \hline      
         \textbf{10 KB}      & {\bf 1166.30}        &\textbf{2.33}           &{\bf 1163.97}           &  {\bf 0.19\%}    & {\bf 0.18}     &{\bf 41.94}   & {\bf 7.75}  \\
        \hline    
    \end{tabular}
\caption{5 seconds block generation interval setting} \label{tab:5sec}
\end{table}
\fi









Varying no




\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
          \textbf{Settings} & \textbf{Case \rom{1}} & \textbf{Case \rom{2}} & \textbf{Case \rom{3}} & \textbf{Case \rom{4}} & \textbf{Case \rom{5}} & \textbf{Case \rom{6}} & \textbf{Case \rom{7}}\\ 
        \hline
          \textbf{Node} 	  & \textbf{6 M} 		  & \textbf{12 M}		  & \textbf{18 M} 		  & \textbf{36 M} 		  & \textbf{54 M} 		  & \textbf{72 M} 		  & \textbf{90 M} \\
          \textbf{Setup}	  & \textbf{83 T} 		  & \textbf{166 T} 	   	  & \textbf{250 T} 		  & \textbf{500 T} 		  & \textbf{750 T}		  & \textbf{1000 T} 	  & \textbf{1250 T} \\
         \hline
          \textbf{Hash Power} & \textbf{1H} 	  	  & {\bf 2H}		 	  & {\bf 3H} 		      & \textbf{6H} 		   &{\bf 9H}  	 		    &{\bf 12H}	   		    &{\bf 15H}   \\
       \hline
       \textbf{Block }   & & & & & & &\\
        \textbf{Generation } &\textbf{3 mins}		& {\bf 1.5 min}	 	      & {\bf 1 min}	 		  &\textbf{30 secs}  	   &{\bf 20 secs}  		  &{\bf 15 secs} 		  &{\bf 12 secs}  \\		
        \textbf{Interval}& & & & & & &\\
       \hline
    \end{tabular}
\caption{Fixed difficulty settings} \label{tab:fixedDifficultySettings}
\end{table}


\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Delay(s)}	    & \textbf{(Kbps)} & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{29.96}     &\textbf{0}	   &\textbf{29.96}    &  {\bf 0\%}	    &\textbf{7.85}           &{\bf 44.17}      & {\bf 9.86}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{76.67}     &\textbf{1.33}	   &\textbf{75.34}	  &  {\bf 1.73\%}	 &\textbf{7.97}          &{\bf 88.9}       & {\bf 25.11}\\
         \hline
         \textbf{Case \rom{3}}  & \textbf{101.29}     &\textbf{1.8}	    &\textbf{99.49}	  &  {\bf 1.77\%}	 &\textbf{8.07}          &{\bf 134.51}     & {\bf33.16}\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{177.67}     &\textbf{20.59}	    &\textbf{157.08}	  &  {\bf 11.52\%}	  &\textbf{41.19}     &{\bf 1168.86}& {\bf 52.36}\\
         \hline 
         \textbf{Case \rom{5}}	& \textbf{237.18}     &\textbf{32.90}	    &\textbf{204.28}	  &  {\bf 13.87\%}	  &\textbf{147.13}     &{\bf 3485.49}& {\bf 68.09}\\
         \hline 
         \textbf{Case \rom{6}} 	& \textbf{216.45}     &\textbf{39.39}	    &\textbf{177.06}	  &  {\bf 18.2\%}	  &\textbf{291.87}     &{\bf 5791.87}& {\bf 59.02}\\
         \hline 
         \textbf{Case \rom{7}}  & \textbf{211.98}     &\textbf{47.55}	    &\textbf{164.43}	  &  {\bf 22.43\%}	  &\textbf{498.97}     &{\bf 8265.55}& {\bf 54.81}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3 - Fixed difficulty setting} \label{tab:case3.1}
\end{table}









\iffalse
%Req analysis ten kontrol et, bi kismi orda artik.
\textbf{IoT devices as blockchain peers} We propose the use of different roles as blockchain peers for IoT devices, considering resource heterogeneity of IoT device ecosystem.
To do so, we propose to use two main roles \textbf{full peers} and \textbf{light peers}. 
As such, IoT devices as full peers will be responsible for transaction validation, block generation, participating in consensus and maintaining all or recent block of the local blockchain.
Whereas light peers, will likely to be able to only receive and send transactions to other devices. 
IoT devices that have limited resources, like CPU power, memory and bandwidth will participate in blockchain networks as light peers, since participation in resource intensive operations like consensus might overwhelm the device. 
For example, IoT devices like Arduino Yun\footnote{store.arduino.cc/arduino-yun} can be used for monitoring and performing basic operations, can take the light peer role, where more advanced devices like Raspberry Pi 3 B \footnote{raspberrypi.org/products/raspberry-pi-3-model-b/}, that are able to perform more resource intensive tasks, may take the full peer role. 
Two main roles, full and light peers, might be diversified by regulating resource usage and participation to the blockchain operations. 
Today's blockchain protocols offers different client models for their protocols, like in Bitcoin as full clients and thin clients\footnote{www.en.bitcoin.it/wiki/Clients}, which we adopted to our Bitcoin emulation to evaluate resource need in Section \ref{sec:emulation}.  
\fi



smartness - device -smartness level

....
In IoT domain, device capabilities are extremely heterogeneous.
To group IoT devices on some common blocks, we refer to the device classification based on their capabilities as presented in \cite{ourPaper2}.
In \cite{ourPaper2}, smartness of the IoT devices, aka smart objects, have been classified into three smartness levels as; first, second, and third smartness levels.
In the following, we examine how IoT devices that are classified into different smartness levels can be part of the blockchain. 


\textbf{First smartness level -- Sensors}\label{sec:firstLevelDevice} 
At the first level, devices have a very limited capacity, being able only to act as  basic sensors, for sensing data from the environment.   
Sensors can not process data, whereas they periodically sense the raw data and send it to the cloud or central data processors like Complex Event Processing (CEP) systems.
Thus, such devices can not be peers in the blockchain network. 
The ideal way to somehow connect those devices to the blockchain network is connecting them to other devices that are peers of the blockchain network. 
If we consider many sensors that are continuously sensing raw data, storing all raw data in the blockchain will be a big hurdle against scalability of the blockchain system.
Therefore, raw data sent by sensors should be processed by higher capability devices or data processing systems that are peers of the blockchain network.
Sensor data needs to be stored in the cloud or servers.
Peers, however, may form transactions and send it to the blockchain network after data processing, if required.
Given all, devices with first smartness level can not directly participate in blockchains, but they can connect to smarter intermediary device indirectly participate.

\textbf{Second smartness level -- Devices with low capabilities}\label{sec:secondLevelDevice} 
At the second level, devices have a limited capacity and computing power, making them able only to  perform basic operations by their own (e.g if/else conditions, sum, multiply).
For example, Arduino Yun\footnote{store.arduino.cc/arduino-yun} can be categorized as a device with second level smartness.
Those devices are able to run basic operating systems such as Alpine Linux\footnote{alpinelinux.org}, and they can connect to the blockchain network.
As such devices run am operating systems and able to process data, they can participate in the blockchain network by performing some simple tasks, like sending transactions.
In parallel with that, today's blockchain protocols offer simple client models.
For example, in case of Bitcoin, nodes can participate in the network as \textit{thin clients}\footnote{$en.bitcoin.it/wiki/Thin_Client_Security\#Thin_Clients$}.
Thin clients perform simpler operations like sending transactions and thus require less resources. 
As such, thin clients do not download all blockchain but they download a complete copy of the headers for all blocks in the entire blockchain and they do not participate in the consensus process.
Given all, devices with second smartness level can take simple client roles that do not require to mine blocks are participate in consensus process, like thin client role in case of Bitcoin. 


\textbf{Third smartness level -- Devices with high capabilities}\label{sec:thirdLevelDevice} 
At the third level, devices have enough capacity and computing power for performing more complex operations by their own.
For example, Raspberry Pi Model B\footnote{raspberrypi.org/products/raspberry-pi-1-model-b} can be categorized as a device with third level smartness.
Those devices run more advanced operating systems like Raspbian\footnote{www.raspbian.org}, and they are able to connect and participate in the blockchain network. 
Such devices can perform more complex blockchain tasks than devices with lower smartness level, such as mining blocks and taking part in the consensus process. 
However, their capabilities are not enough to solve very complex PoW puzzles to mine a block, or propagate big blocks.
For example, in case of Bitcoin, Raspberry Pi Model B has 0.2 mega hash per second (0.2 MH/s) and with the difficulty setting in Bitcoin network in late 2017, it would take more than 1000 years to solve the PoW puzzle for a million Raspberry Pi Bs.
Moreover, their bandwidth capabilities are limited, therefore very big block sizes or very short block generation interval settings are not suitable for such devices (as discussed in Evaluation \rom{1}).
Given all, devices with the third level of smartness can participate in the blockchain networks as full peers, by carefully setting consensus parameters and blockchain rules such as block size and block generation interval.





























\textbf{Smart contract concept}  Today, some blockchains use an important concept referred to as "smart contracts". This refers to executable scripts stored in blockchain. The smart contract concept was first introduced in \cite{szabo} as 'a computerized transaction protocol that executes the terms of a contract'. More specifically, smart contracts are deterministic self-executing contractual clauses. Once a smart contract is deployed on a blockchain it is stored forever with the following properties: nobody can control or modify it, it has a unique address. Since smart contracts can not be modified throughout their existence on the blockchain, every peer in the network can trust them. They have unique address on the blockchain, and its clauses can be triggered by peers, by sending transactions to execute them. Smart contracts describe  outcomes of the contract execution and allows us to express business logic inside the blockchain \cite{scForIoT}, which opens up an opportunity for IoT applications.



%d
\subsection{Mining Cartel Attack (51\% attack}\label{sec:51attack}
In mining cartel attack, attacker gathers massive hashrate, that is bigger than 50\% of the total mining power of the devices in the system \cite{miningCartel}.
In performing such attack, and will be able to control the network. 
As such, as long as attacker maintains majority of the mining power in the system, attacker can prevent others to generate new blocks, prevent other devices' transactions to make into blocks.
This attack is a huge threat against robustness of the blockchain, as attacker is able to perform malicious activities and can not be stopped by honest devices.
In our architecture, we suggest to use of consortium or private blockchains (cfr. to Section\ref{sec:background} for more information) would limit this attack factor, as only selected devices can contribute to the block mining process.
However, attacker may compromise devices that are authorized to generate block and if he/she has gathers majority of the mining power, can launch this attack.
We discuss device device compromise attacks in Section \ref{sec:deviceComp}.
In case of mining cartel attack on private or consortium blockchain, firstly, administrators of the blockchain should identify infected devices that are generating malicious transactions and blocks.
Then, honest devices should not propagate blocks and transactions that are sent by infected devices and they should be forced drop their connections to malicious devices.
Finally, the blockchain have to be diverted to the latest correct state before the launching of the attack in all devices by deleting malicious blocks.




%d
\subsection{Device compromise attacks}\label{sec:devComp}
In performing device compromise attacks, attacker subversively gains access to an IoT device, where he can drop the device from the network and may control it to perform malicious activities.
Major threats on blockchains systems related to node compromise attacks are \textit{device capture} and \textit{device controlling}. 
By performing device capture attack, attacker may drop the device from the blockchain network.
In which, device is unable to participate in the network as such; it can not processes data and generate transactions, propagate and check correctness of the blocks and transactions sent by its peer devices.  
Whereas in performing device controlling attack, an attacker may send malicious transactions and blocks, or he/she may use compromised devices to launch other types of attacks, such as mining cartel attack, or Denial of Service (DoS) attack.
IoT devices should be complemented with authentication and authorization mechanisms (see e.g., \cite{authorizationIoT}) and strong passwords to hinder attacker's access to devices.
However, some IoT devices have very limited resources (devices within the first smartness level, see Section \ref{sec:Background}), and they may not be suitable to be complemented with authorization and authentication mechanism.
To cope with device compromise attacks on low level devices, IoT devices with higher capabilities (devices within the third smartness level) should be complemented with intrusion detection systems (see e.g., \cite{intrusionSvelte}, \cite{adversaryNodeCapWSN})  so as  to make them able to analyze the network and detect compromised devices and drop connections.  




%d
\subsection{Sybil attacks}
Sybil attacks refer to maliciously manipulating IoT systems with many sybil IoT devices that are generated with stolen and fabricated identities \cite{sybilDefenceEvaluation}. 
In performing sybil attacks, an attacker node claims several stolen identities, and attempts to fill the blockchain network with clients controlled by him.
In blockchain systems, honest IoT devices may only be connected to sybil devices controlled by the attacker.
Sybil attacks can be performed to disseminate spam and malware to honest smart objects \cite{sybilIoT}.
In PoW blockchains, to generate a block what matters is the computational power, but not the number of entities by count.
In which, as long as attacker has the limited mining power, he would not be able to produce more blocks by generating creating several identities as he distributes his mining power to the his sybil identities.
However, launching a sybil attack can be helpful in executing other attacks, such as network partitioning and eclipse attacks\footnote{www.en.bitcoin.it/wiki/Weaknesses} , that are discussed in Section \ref{sec:networkEclipse}.
In which, by launching sybil attack, victim device would likely to be connected to sybil nodes, thus it gets disconnected from the network. 
By doing that attacker may generate partition the network, or can try to send bogus blocks or transactions to the victim node. 

In IoT domain, various approaches have been proposed to deal with sybil attacks, such as cryptography based approaches \cite{sybilCryptography}, intrusion detection approaches \cite{intrusionSvelte}, or network based approaches making use of RSS readings \cite{rssiSybil,sybilDetection}. 
In order to cope with sybil attacks, IoT devices should be complemented with an hybrid prevention setting, that makes use of both intrusion detection and RSS readings based approaches. 
In particular, IoT devices within third smartness level can be complemented with intrusion detection systems \cite{intrusionSvelte} to detect sybils, as we assume they are honest and have enough resources to host intrusion detection systems. 
Whereas, all IoT devices objects will be complemented with RSS readings based approach \cite{rssiSybil,sybilDetection}, as they offer efficient solutions for resource constrained devices.
Such approaches define a threshold value on RSS readings to distinguish legitimate and sybil nodes based on nodes’ behavior in the network.
In our architecture, we propose to distribute IoT devices into different blockchains by considering their geographical locations to be as close to each other as possible. 
In which, IoT devices will maintain lists of devices and RSS values of devices that are in their coverage area, and they will define a threshold value to detect sybil devices.

%If there is a discrepancy between the amount of work that the two connected nodes claim, then a client knows that the one with the least work is probably doing something malicious, lying.
%providing white-listed devices to the peers; before connecting to the new peer, IoT device should ask for some information from its local blockchain like current difficulty, or information about transactions  or blocks that have been in longest chain for a long time.





%d
\subsection{Network partitioning and Eclipse attacks}\label{sec:networkEclipse}
%eclipse
In eclipse attack on the blockchain systems \cite{eclipseAttack}, attacker monopolizes all of the victim devices' incoming and outgoing connections to the other devices (e.g., 117 to 8 in Bitcoin).
The IP addresses to which the victim IoT device connects are blocked or diverted towards an adversary devices \cite{eclipseAttack}.
Attacker can hold multiple IP addresses, such as by performing sybil attack,and spoof the victim IoT devices from the network.
If all connections of an IoT device are with attacker's malicious devices, attacker may send false blocks and transactions to target IoT devices where victim device have to accept if they are in consistence with device's local blockchain.
However attacker can not force target IoT devices to accept something that network hasn't agreed upon before.


%partitioning
Attacker may try to eclipse set of devices from the rest of the network to generate partitions in the network, referred as network partitioning attack.
In performing network partitioning attack, attacker aims to completely disconnect a set of nodes from the network such that there is no active connection between them \cite{routingAttacks}.
To partition the network, attacker either eclipse victim devices by divert all connections to his sybil identities, or he should cut all the connections by dropping any packets to or from victim device set.
This attack cause to generate more than one subnetworks, where devices in the disjoint parts will have different views of the blockchains and recent transactions.
In which, total hash power of the system will reduce, and victim devices will be forced to waste computational power and energy on obsolete views of blockchain and it might damage correct execution of IoT applications.


%defence
In order to prevent these attacks, IoT devices should be complemented with an hybrid prevention setting, that makes use of both includes white-listed devices method and intrusion detection approach. 
Firstly, IoT devices within third smartness level can be complemented with intrusion detection systems \cite{intrusionSvelte} in order to detect misbehaving devices. 
Moreover, IoT devices should have a list of devices, aka white-listed devices, to store the addresses of trustworthy devices \cite{routingAttacks}. 
Trustiness of the devices should be changed according to activities of the device, in which misbehaving devices detected by intrusion mechanism should be updated as untrusted device, its' connections should be dropped. 







\subsection{Man in the middle (MITM) attack}
In performing attacks targeting communication between IoT devices on blockchain infrastructure, attacker may aim to position herself in between two parties to alter communication by changing transactions and blocks, or to slow down block propagation. Major threats of MITM attack to proposed mechanism are \textbf{data tampering} and \textbf{slowing information propagation}.

\textbf{Data tampering} This attack aims to violate integrity of the transaction by tampering with its data. As discussed in Section \label{sec:background}, blockchain protocols use digital signature algorithms, specifically Elliptic Curve Digital Signature Algorithm (ECDSA) to cryptographically sign transactions sent among peers. Public keys of the users published across all peers of the network and their integrity is protected through stored blocks. In blockchain protocols, transactions should have signatures that are specific to each transaction. If attacker does not have the private key of the original sender of the transaction, it is infeasible for her to generate valid signature, since validity of the signatures can be checked by public keys known by all peers. Therefore, proposed architecture does not allow tampering of transaction information between IoT devices.

\textbf{Block witholding} 
\cite{tamperingDelivery}
.
Tampering: In a Bitcoin network, after mining a block the miners broadcast the information about newly mined blocks. New transactions will be broadcast from time to time in the network. The network assumes that the messages will reach to the other nodes in the Bitcoin network with a good speed. However, authors in [64] ground this assumption, and they prove that the adversary can induce delays in the broadcast packets by introducing congestion in the network or making a victim node busy by sending requests to all its ports. Such type of tampering can become a root cause for other types of attacks in the network.
.
By slowing information propagation, attacker aims to generate inconsistency inside blockchain network. We discuss effects and how to defend system against such attack in Section \ref{sec:networkEclipse}.
.
 In performing \textbf{propagation delay attack}, attacker aims to generate inconsistency inside blockchain network by trying to make peers having different views of current state of the blockchain, in order to perform malicious activities.  
.
Propagation delay attack may also effect victim's view on current state of the blockchain, and may cause inconsistency to victim's operations.
.

\textbf{Transaction hiding:}








\subsection{Denial of service (DoS) attacks}
In general, DoS attacks may cause \textit{unavailability} of a subnet of IoT devices, by disrupting their resources and blocking valid requests and communication among devices. Proposed architecture can be  target of two types of DoS attacks as \textbf{DoS attacks targeting IoT devices} and secondly \textbf{DoS attacks targeting blockchain infrastructure}. 

%Buna gerek yok.
\textbf{DoS attacks targeting IoT devices} An attacker may perform DoS attack against IoT devices to interrupt correct execution of the IoT application and to capture the device. Moreover, effects of this attack to blockchain infrastructure depends on ratio of hashing power of victim devices to total hashing power of the blockchain network. If victim devices participate in private/consortium blockchain, such attack will not threat data integrity of blockchain, and new transactions generated by other devices can be executed correctly by remaining honest nodes. However, if honest target devices are participate in a public blockchain infrastructure, decrease of honest hashing power against rest of the nodes which might be malicious. In case malicious nodes become majority, they can perform 51\%attack that we discuss in the following Section \ref{sec:51attack}. We propose to use of strong authentication and authorization mechanisms on IoT devices an preventive mechanisms (e.g. \cite{ddosPreventiveIoT}, \cite{preventiveAdapDDoS}) against DoS attacks.   

\textbf{Dos attacks targeting blockchain infrastructure} An attacker may perform DoS attack against blockchain infrastructure using her malicious blockchain nodes in the network. 
Such attack is only effective against public blockchains, where anyone can participate in the network \footnote{We assume in private blockchains all peers are monitored closely by system administrators and if attacker compromise an IoT device and perform malicious activities, it can be detected easily and removed from the blockchain network}. 
Attacker may target to cause unavailability of system, by preventing processing of transactions honest peers, or attacker may try to keep honest peers busy with his transactions to waste their resources thus interrupt correct execution of the blockchain network. As such, this attack may cause double spend transactions to succeed, may generate delays on block and transaction propagation or may prevent valid transactions to be mined into the new blocks.
\subsubsection{DoS Attack Evaluation}\label{sec:dosEvaluation}
We have performed some Dos vectors targeting blockchain infrastructure by using Bitcoin protocol, and we have referred to Bitcoin stress test analysis in \cite{bitcoinStressTesting} for attack vectors. We have performed 4 different DoS attack vectors on emulated IoT devices that participate in Bitcoin network. In following, first we discuss our emulation settings then we present evaluated attacks and we discuss their their effects to the proposed architecture and how to protect against such attacks.

\subsubsection{DoS Attack Experimentation Structure}\label{sec:attackEmuStructure}
In our evaluations, we have emulated the victim IoT device using LXC system container tool. Emulated IoT devices run Ubuntu 16.04 (Xenial) operating system\footnote{releases.ubuntu.com/16.04/}. We have configured the victim IoT device with 512 MB of RAM and 50\% of one core of Intel Core i7 2.70 GHz CPU. We have used Bitcoin protocol's full node model for the victim IoT device, using bitcoind version 14.02. In order to attack emulated victim IoT device, we have emulated 10 attacker IoT devices using LXC system container tool, which run Alpine Linux operating system version 3.6.0. We set RAM limit of light peers to 128 MB, and limited CPU usage to 20\% of one core of Intel Core i7 2.70 GHz CPU. In order to perform DoS attacks on victim IoT device, we have developed attacker clients that run on attacker IoT devices. We have set Java SE, JRE 8 update 131 environment to our attacker IoT devices, and, we have developed attacker client applications with bitcoinj library using Java SE, JDK version 8 Update 131. All of our evaluations have been run on regtest network of Bitcoin protocol. 

\subsubsection{Sending many valid transactions} 
This DoS vector aims to overwhelm IoT device by increasing it's CPU usage, since peers of the blockchain networks have to check correctness of the transaction and if valid adding transaction to its memory. We have emulated the victim IoT device and 10 attacker IoT devices with configurations given in Section \ref{sec:attackEmuStructure}. In our experiments, attacker IoT devices continuously sent transactions directly to the victim device, the victim device has to check correctness of transactions and put into its memory if they are valid. We have performed to attack for 30 minutes, where in total 65000 transactions with one input (attacker node's account address) and one output address, sent to the victim device. We present CPU overhead of the victim node caused by this attack vector in Figure \ref{fig:validTXs}, in which when attack started (around 15.01 in given figure) CPU usage increased significantly until attack has been terminated (around 15.31 in given figure). As such, 10 attacker IoT devices with previously given configurations, in average, managed to consume 35\% of the CPU power of the victim IoT device. Additionally, such attack generated 16 MB overhead to RAM usage of the victim IoT device.

\begin{figure} 
    \centering
  \subfloat[CPU Utilization DoS]{%      
     \includegraphics[width=\linewidth]{figures/DoS_Valid_CPU_Utilization.png}}
  	  \label{1a}\hfill 
  \caption{Presents CPU utilization of IoT peer DoSed with valid TXs}
  \label{fig:validTXs} 
\end{figure}
In proposed architecture, this attack may drop IoT devices from blockchain network by causing DoS. In order to decrease possibility of successful attack, number of transactions that can be received from one peer in a period should be limited regrading resources of the IoT devices participating in the network. Additionally, this attack comes with its cost in Bitcoin network, since attacker needs to pay transaction fee for each transactions, therefore applying a transaction fee can also reduce chances for successful attack. 

\subsubsection{Sending many invalid transactions} 
This DoS vector aims to overwhelm victim IoT device increasing its CPU usage. As such, we have evaluated this attack vector on Bitcoin network by continuously sending invalid transactions with one input and one output addresses, from 10 emulated attacker IoT devices to the victim IoT device. Attacker IoT devices continued to attack to the victim IoT device around 20 minutes, where we continuously send may invalid transactions. We present CPU overhead of the victim node caused by this attack vector in Figure \ref{fig:invalidTXs}, in which when attack started (around 09.50 in given figure) CPU usage increased significantly until attack has been terminated (around 10.10 in given figure). In given configurations with 10 attacker nodes, in average, attacker devices managed to consume 53\% of the CPU power of the victim IoT device.

\begin{figure} 
    \centering
  \subfloat[CPU Utilization DoS]{%      
     \includegraphics[width=\linewidth]{figures/DoS_Invalid_CPU_Utilization.png}}
  	  \label{1a}\hfill 
  \caption{Presents CPU utilization of IoT peer DoSed with invalid TXs}
  \label{fig:invalidTXs} 
\end{figure}

In proposed architecture, this attack may drop IoT devices from blockchain network by causing DoS. In order to decrease possibility of successful attack, connection to the peer that send invalid transactions should be dropped. 


\subsubsection{Sending big transactions} 
This attack vector aims to overwhelm victim IoT device, since larger transactions including more operations requires IoT device's CPU and RAM usage. We have tested this attack vector by trying to send transactions from one attacker IoT device with increased transaction size, by adding many output addresses to the victim IoT device. As such, we have evaluated this attack vector on Bitcoin network by trying to generate and release big transactions, that we generate with an Bitcoin application developed using bitcoinj library.  We present our results by showing number of outputs that we put in single transaction, size of the transaction and whether generated transaction could be released into the network  in Table \ref{tab:bigTX}.
\begin{table}[t]
\centering
\caption{Sending Big Transactions}
\begin{tabular}{lllllll}
\hline
No of Output         & \multicolumn{1}{c}{100}  & \multicolumn{1}{c}{250}  & \multicolumn{1}{c}{500}  & \multicolumn{1}{c}{1000}  & \multicolumn{1}{c}{2930}  & \multicolumn{1}{c}{3000}  \\  \hline
TX Size                & \multicolumn{1}{c}{1 KB}    & \multicolumn{1}{c}{10 KB}   & \multicolumn{1}{c}{25 KB}   & \multicolumn{1}{c}{50 KB}   & \multicolumn{1}{c}{99 KB}   & \multicolumn{1}{c}{110 KB}  \\ \hline
Success         & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\checkmark}  & \multicolumn{1}{c}{\textbf{X}}    \\ %\hline
\end{tabular}
\end{table}\label{tab:bigTX} 

As our findings verify, Bitcoin protocol limits maximum size the normal transactions as 100 KB. This attack may increase memory usage of IoT devices on the network, which may drop IoT devices from blockchain network by causing DoS. To decrease success possibility of this attack, maximum size of the transactions should be limited with regards to memory resource constraints of IoT devices on the network.


\subsubsection{Sending many big transactions} 
This attack aims to cause memory overwhelm of victim IoT device, by sending many transactions that each are generating many outputs. We have tested this attack vector by  sending as many transactions as possible from one attacker IoT device with many output addresses to the victim IoT device on Bitcoin network which is configured with the settings given in Section \ref{sec:attackEmuStructure}. In our experiments, we have varied transaction sizes by varying number of output addresses in transactions. We present our results by showing number of outputs that we put in each transaction, size of the transaction, how many transactions with given settings could be sent to the peer and size of the total overhead on memory of the IoT device in Table \ref{tab:manyBigTX}. Bitcoin protocol drops the connection to the attacker node after receiving certain amount of transactions, which we executed many times every attack and presented the average number.
 
\begin{table}[t]
\centering
\caption{Generating Big Transactions}
\begin{tabular}{lllllll}
\hline
No of Output         & \multicolumn{1}{c}{100}  & \multicolumn{1}{c}{250}  & \multicolumn{1}{c}{500}  & \multicolumn{1}{c}{1000}  & \multicolumn{1}{c}{2000}  & \multicolumn{1}{c}{2950}  \\  \hline
TX Size (KB)             & \multicolumn{1}{c}{3.6}    & \multicolumn{1}{c}{8.7}   & \multicolumn{1}{c}{17.1}   & \multicolumn{1}{c}{34.2}   & \multicolumn{1}{c}{68.2}   & \multicolumn{1}{c}{98.8}    \\ \hline
No of TXs        & \multicolumn{1}{c}{296}  & \multicolumn{1}{c}{193}  & \multicolumn{1}{c}{108}  & \multicolumn{1}{c}{63}  & \multicolumn{1}{c}{32}  & \multicolumn{1}{c}{22}  \\  \hline
Total Size (MB)     & \multicolumn{1}{c}{1.06}  & \multicolumn{1}{c}{1.67}  & \multicolumn{1}{c}{1.86}  & \multicolumn{1}{c}{2.15}  & \multicolumn{1}{c}{2.18}  & \multicolumn{1}{c}{2.17}  \\  \hline
\end{tabular}
\end{table}\label{tab:manyBigTX}    
    

This attack may increase memory usage of IoT devices on the network, which may drop IoT devices from blockchain network by causing DoS. Therefore, in order to decrease success possibility of this attack vector, firstly maximum size of the transactions should be limited with regards to memory resource constraints of IoT devices on the network. Secondly, total size of the transactions that can be received from a peer should be limited, and connection to the peer should be dropped by victim peer device.











INTRODUCTION

\iffalse
Traceability: BPIIoT platform can be used for developing traceability applications
for manufactured products. Smart contracts between the consumers and manufac-
turers can keep production records, for example, which factory and which machines
within the factory were used for manufacturing a particular product.
 Supply Chain Tracking: BPIIoT platform can be used for developing supply chain
tracking applications. The Blockchain and Smart Contracts can keep a formal regi-
stry of products and track their possession through different points in a supply
chain. Such applications can also enable automated financial settlements on delivery
confirmations.
Product Certification: BPIIoT platform can be used for developing product certifi-
cation applications. The manufacturing information for a product (such as the ma-
nufacturing facility details, machine details, manufacturing date and parts informa-
tion) can be recorded on the Blockchain. This information can help in proving the
authenticity of the products eliminating the need for physical certificates which can
be prone to tampering and forging.
 Consumer-to-Machine & Machine-to-Machine Transactions: BPIIoT can enable
machine-to-machine transactions for manufacturing services. For example, a con-
sumer can send a request for manufacturing a product by sending a transaction to a
manufacturer's smart contract along with the payment made in a crypto currency
(such as Ethers). The manufacturer’s smart contract can then send transactions to
smart contracts associated with individual machines (consumer-to-machine trans-
actions). If services of different machines are required for manufacturing a product,
the machines can send micro-transactions to other machines (machine-to-machine
transactions).
Tracking Supplier Identity & Reputation: BPIIoT platform can be used for devel-
oping supplier identity and reputation management applications which track vari-
ous performance parameters (such as delivery times, customer reviews and seller
ratings) for sellers. Such applications can be used by consumers to find the sellers
that can meet their manufacturing requirements and by manufacturers for finding
suppliers for consumables. Smart contracts can also help in automatically negotiat-
ing best prices for consumables and supplies in real-time based on the seller reputa-
tions.
Registry of Assets & Inventory: BPIIoT platform can be used for developing ap-
plications for maintaining records of manufacturing assets and inventory. These ap-
plications can keep records of the asset identification information and the transfer
of assets through the supply chain eliminating the need for manual paper records.
On-Demand Manufacturing: The BPIIoT platform will enable a marketplace of
manufacturing services where the machines will have their own Blockchain ac-
counts and the users will be able to provision and transact with the machines di-
rectly to avail manufacturing services in a CBM-like on-demand model. BPIIoT can
enable peer-to-peer networked manufacturing applications where the peers will be
able to avail manufacturing services (such as CNC machining or 3D printing) by
sending transactions to the machines.
Smart Diagnostics & Machine Maintenance: BPIIoT platform can be used for de-
veloping smart diagnostics and self-service applications for machines where the
machines will be able to monitor their state, diagnose problems, and autonomously
place service, consumables replenishment, or part replacement requests to the ma-
chine maintenance vendors. Smart contracts between manufacturers and vendors
for procurement of supplies and service of machines can help in automating the
machine maintenance tasks. We describe the implementation of a smart diagnostics
and machine maintenance application using the proposed platform in Section-7.
\fi
\iffalse
In ADEPT project \cite{ibmadept} of IBM and Samsung, autonomous decentralized peer to peer telemetry platform, IBM aims to achieve scalable and secure IoT systems by using blockchain technology as backbone. The ADEPT architecture consists three peer architectures, where classification is done according to the capabilities of devices (i.e. computational power, memory etc.) namely \textit{light peer} \textit{standard peer} and \textit{peer exchange}. \textit{Light peer} devices are with low level capabilities where they would have no capabilities of storing blockchains, and would only have its own blockchain address and balance inside the device. \textit{Standard peer} devices are capable of holding blockchain information for a certain period of time, where it can retain part of blockchain that is related to it or additionally also be for other \textit{light peer} devices in its ecosystem. \textit{Peer exchange} are high end devices with strong computing and storage capabilities; and able to  store blockchain, host marketplaces, demand supply chains etc.
\fi
%as its happening quite frequently lately \footnote{mirai, etc.},
%Moreover, considering high heterogeneity of IoT devices \cite{Whitmore2014}, enabling them to cooperate and generating a smooth execution environment is not an easy task. 
%Key objectives of the project are: accomplishing foundational IoT process tasks without centralized control infrastructure; having   robust security for transaction processing, storage, transport; and providing privacy by design. 
%ADEPT has been implemented using three protocols: TeleHash for peer to peer messaging among IoT devices, BitTorrent for file sharing, and Ethereum for blockchain and smart contracts. 
%Key element of the blockchain technology is an append-only, distributed and replicated ledger, where every transaction is recorded, and  cryptography techniques are used to  ensure data integrity, after achieving consensus on current state of the blockchain among peers 
\iffalse
@misc{buterinblockchainprivacy,
 author = {Vitalik Buterin},
 title = {{Privacy on the Blockchain}},
 howpublished = "\url{https://blog.ethereum.org/2016/01/15/privacy-on-the-blockchain}",
 year = {2015}, 
 note = "[Online; accessed 10-December-2016]"
}  
\fi














\iffalse
\subsubsection{Fixed difficulty}\label{sec:eva3.1}
We have varied block generation intervals from 3 minutes to 12 seconds with direct proportion to the number of devices on fixed block generation difficulty.  
Evaluation settings have been presented in Table \ref{tab:noDeviceSettings} and experiment results  in Table \ref{tab:case3.1Neds}, \ref{tab:case3.1Europe} and \ref{tab:case3.1World}.
.
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
          \textbf{Settings} & \textbf{Case \rom{1}} & \textbf{Case \rom{2}} & \textbf{Case \rom{3}} & \textbf{Case \rom{4}} & \textbf{Case \rom{5}} & \textbf{Case \rom{6}} & \textbf{Case \rom{7}}\\ 
        \hline
          \textbf{Node} 	  & \textbf{6 M} 		  & \textbf{12 M}		  & \textbf{18 M} 		  & \textbf{36 M} 		  & \textbf{54 M} 		  & \textbf{72 M} 		  & \textbf{90 M} \\
          \textbf{Setup}	  & \textbf{83 T} 		  & \textbf{166 T} 	   	  & \textbf{250 T} 		  & \textbf{500 T} 		  & \textbf{750 T}		  & \textbf{1000 T} 	  & \textbf{1250 T} \\
         \hline
          \textbf{Hash Power} & \textbf{1H} 	  	  & {\bf 2H}		 	  & {\bf 3H} 		      & \textbf{6H} 		   &{\bf 9H}  	 		    &{\bf 12H}	   		    &{\bf 15H}   \\
       \hline
       \textbf{Block }   & & & & & & &\\
        \textbf{Generation } &\textbf{3 mins}		& {\bf 1.5 min}	 	      & {\bf 1 min}	 		  &\textbf{30 secs}  	   &{\bf 20 secs}  		  &{\bf 15 secs} 		  &{\bf 12 secs}  \\		
        \textbf{Interval}& & & & & & &\\
        \hline
    \end{tabular}
\caption{Hash power experiments settings} \label{tab:noDeviceSettings}
\end{table}
.
.
In all cases, increasing number of devices cause longer block propagation delays, which in turn increase stale block generation rates and decrease transaction throughputs.
Shorter block generation intervals cause system to produce more blocks.
However, due to higher number of devices and longer block propagation delay, stale block generation rates increase.
%Netherlands setting can achieve 25.11 transaction throughput
.
%1. case Netherlands 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Delay(s)}	    & \textbf{(Kbps)} & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{29.96}     &\textbf{0}	   &\textbf{29.96}    &  {\bf 0\%}	    &\textbf{7.85}           &{\bf 44.17}      & {\bf 9.86}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{76.67}     &\textbf{1.33}	   &\textbf{75.34}	  &  {\bf 1.73\%}	 &\textbf{6.97}          &{\bf 88.9}       & {\bf 25.11}\\
         \hline
         \textbf{Case \rom{3}}  & \textbf{101.29}     &\textbf{2}	    &\textbf{99.29}	  &  {\bf 1.97\%}	  &\textbf{8.07}     &{\bf 134.51}& {\bf33.09 }\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{177.67}     &\textbf{20.59}	    &\textbf{157.08}	  &  {\bf 11.52\%}	  &\textbf{41.19}     &{\bf 1168.86}& {\bf 52.36}\\
         \hline 
         \textbf{Case \rom{5}}	& \textbf{237.18}     &\textbf{32.90}	    &\textbf{204.28}	  &  {\bf 13.87\%}	  &\textbf{147.13}     &{\bf 3485.49}& {\bf 68.09}\\
         \hline 
         \textbf{Case \rom{6}} 	& \textbf{216.45}     &\textbf{39.39}	    &\textbf{177.06}	  &  {\bf 18.2\%}	  &\textbf{291.87}     &{\bf 5791.87}& {\bf 59.02}\\
         \hline 
         \textbf{Case \rom{7}}  & \textbf{211.98}     &\textbf{47.55}	    &\textbf{164.43}	  &  {\bf 22.43\%}	  &\textbf{498.97}     &{\bf 8265.55}& {\bf 54.81}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.1: Netherlands setting} \label{tab:case3.1Neds}
\end{table}
%2. case Europe 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Delay(s)}	    & \textbf{(Kbps)} & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{36.8}     &\textbf{0}	    &\textbf{36.8}	  &  {\bf 0\%}	  &\textbf{9.57}     &{\bf 44.6}& {\bf 12.26}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{62.49}     &\textbf{2.99}	    &\textbf{59.5}	  &  {\bf 4.78\%}	  &\textbf{8.91}     &{\bf 90}& {\bf 19.63}\\
         \hline
         \textbf{Case \rom{3}}  & \textbf{100.12}     &\textbf{5.2}	    &\textbf{94.92}	  &  {\bf 5.19\%}	  &\textbf{10.01}     &{\bf 138.76}& {\bf 31.64}\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{176.55}     &\textbf{21.29}	    &\textbf{155.26}  &  {\bf 12.05\%}	  &\textbf{38.03}     &{\bf 1051.63}& {\bf 51.75}\\
         \hline 
         \textbf{Case \rom{5}}	& \textbf{227.01}     &\textbf{46.61}	    &\textbf{180.4}	  &  {\bf 20.53\%}	  &\textbf{201.8}     &{\bf 3755.05}& {\bf 60.1}\\
         \hline 
         \textbf{Case \rom{6}} 	& \textbf{212.1}     &\textbf{49.51}	    &\textbf{172.59}	  &  {\bf 23.34\%}	  &\textbf{331.54}     &{\bf 6125.58}& {\bf 57.53}\\
         \hline 
         \textbf{Case \rom{7}}  & \textbf{212.19}     &\textbf{55.08}	    &\textbf{157.11}	  &  {\bf 25.95\%}	  &\textbf{558.93}     &{\bf .}& {\bf 52.37}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.1: Europe setting} \label{tab:case3.1Europe}
\end{table}
%3. case World 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{Setting}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Case}          &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{}              & 				     &   			   & 			      &                 &\textbf{Delay(s)}	    & \textbf{(Kbps)} & \\
         \hline
         \textbf{Case \rom{1}}  & \textbf{32}     &\textbf{0.65}	    &\textbf{31.35}	  &  {\bf 2.03\%}	  &\textbf{10.13}     &{\bf 45.45}& {\bf 10.45}\\
         \hline
         \textbf{Case \rom{2}}  & \textbf{58.74}     &\textbf{3.62}	    &\textbf{55.12}	  &  {\bf 6.1\%}	  &\textbf{10.22}     &{\bf 91.27}& {\bf 18.37}\\
         \hline
         \textbf{Case \rom{3}}  & \textbf{98.29}     &\textbf{9.13}	    &\textbf{89.16}	  &  {\bf 9.28\%}	  &\textbf{13.01}     &{\bf 142.90}& {\bf 29.72}\\
         \hline 
         \textbf{Case \rom{4}}  & \textbf{174.87}     &\textbf{28.17}	    &\textbf{146.7}	  &  {\bf 16.1\%}	  &\textbf{40.99}     &{\bf 1025.21}& {\bf 48.9}\\
         \hline 
         \textbf{Case \rom{5}}	& \textbf{215.84}     &\textbf{43.7}	    &\textbf{172.14}	  &  {\bf 20.24\%}	  &\textbf{190.05}     &{\bf 3794.63}& {\bf 57.38}\\
         \hline 
         \textbf{Case \rom{6}} 	& \textbf{209.55}     &\textbf{50.62}	    &\textbf{158.93}	  &  {\bf 24.15\%}	  &\textbf{369.25}     &{\bf 6555.25}& {\bf 52.44}\\
         \hline 
         \textbf{Case \rom{7}}  & \textbf{198.88}     &\textbf{57.12}	    &\textbf{141.66}	  &  {\bf 28.72\%}	  &\textbf{574.35}     &{\bf 11284.13}& {\bf 47.22}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.1: World setting} \label{tab:case3.1World}
\end{table}
.
.
.
.
.
\subsubsection{Varying difficulty}\label{sec:eva3.2}
We have varied number of IoT devices on fixed 1 minute block generation interval setting.
In which, difficulty of the PoW puzzle has been varied according to number of miners in the blockchain.
Evaluation results have been presented  in Table \ref{tab:case3.2Neds}, \ref{tab:case3.2Europe} and \ref{tab:case3.2World}.
.
In all evaluation cases, increasing number of devices cause to increase in block propagation delays, as every device have to check and propagate generated blocks.
In parallel,  stale block generation rates and lower transaction throughputs have been observed.
Netherlands case has the lowest stale block generation rates, due to low network latency.
In which, Netherlands setting complies with the integration metrics with up to 250 peers with given settings, whereas World setting does not comply with the metrics for any case due to high stale block rates. 
%1. case Netherlands 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{No of}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Miners/}     &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{Total}       & 				   &   			     & 			        &                 &\textbf{Delay(s)}	  & \textbf{(Kbps)} & \\
         \hline
         \textbf{6/83}        & \textbf{96.13}    &\textbf{0}       &\textbf{96.13}	    &  {\bf 0\%}	  &\textbf{9.38}          &{\bf 135.76}        & {\bf 32.04}\\
         \hline
         \textbf{12/166}    & \textbf{97.29}    &\textbf{0.33}	   &\textbf{96.96}	  &  {\bf 0.33\%}	 &\textbf{7.07}           &{\bf 133.37}       & {\bf 32.32}\\
         \hline         
         \textbf{18/250}    & \textbf{99.32}    &\textbf{1.78}	   &\textbf{96.65}	  &  {\bf 1.79\%}	 &\textbf{10.07}           &{\bf 136.37}       & {\bf 32.21}\\
         \hline 
         \textbf{36/500}    & \textbf{103.03}    &\textbf{4.42}	   &\textbf{98.61}	  &  {\bf 4.29\%}	 &\textbf{19.41}        &{\bf 122.99}       & {\bf 32.86}\\
         \hline  
         \textbf{54/750}    & \textbf{93.41}    &\textbf{4.49}	   &\textbf{88.92}	  &  {\bf 4.8\%}	 &\textbf{13.61}        &{\bf 102.03}       & {\bf 26.97}\\
         \hline 
         \textbf{72/1000}   & \textbf{93.03}    &\textbf{3.42}	   &\textbf{89.61}	  &  {\bf 3.67\%}	 &\textbf{19.41}        &{\bf 122.99}       & {\bf 32.86}\\
         \hline 
         \textbf{90/1250}   & \textbf{92.77}    &\textbf{2.98}	   &\textbf{89.78}	  &  {\bf 3.21\%}	 &\textbf{15.67}        &{\bf 107.01}       & {\bf 29.92}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.2: Netherlands setting} \label{tab:case3.2Neds}
\end{table}
%2. case Europe 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{No of}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Miners/}     &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{Total}       & 				   &   			     & 			        &                 &\textbf{Delay(s)}	  &\textbf{(Kbps)} & \\
         \hline
         \textbf{6/83}       & \textbf{105.97}    &\textbf{0.94}     &\textbf{105.93}	&  {\bf 0.88\%}	  &\textbf{12.88}        &{\bf 147.79}       & {\bf 35.31}\\
         \hline
         \textbf{12/166}     & \textbf{84.01}    &\textbf{1.64}	     &\textbf{82.37}	&  {\bf 1.95\%}	 &\textbf{8.40}          &{\bf 135.58}       & {\bf 27.45}\\
         \hline         
         \textbf{18/250}     & \textbf{100.03}   &\textbf{8.15}	     &\textbf{91.88}	&  {\bf 8.14\%}	 &\textbf{12.05}         &{\bf 146.13}       & {\bf 30.62}\\
         \hline 
         \textbf{36/500}     & \textbf{104.14}   &\textbf{7.89}	    &\textbf{96.25}	    &  {\bf 7.57\%}	 &\textbf{15.39}         &{\bf 148.11}       & {\bf 32.08}\\
         \hline  
         \textbf{54/750}     & \textbf{90.05}    &\textbf{6.38}	   &\textbf{83.77}	    &  {\bf 7.08\%}	 &\textbf{20.46}         &{\bf 168.43}       & {\bf 27.92}\\
         \hline 
         \textbf{72/1000}    & \textbf{97.44}    &\textbf{8.74}     &\textbf{88.70}	    &  {\bf 8.96\%} &\textbf{19.71}         &{\bf 155.68}       & {\bf 28.90}\\
         \hline 
         \textbf{90/1250}    & \textbf{82.78}    &\textbf{5.99}	   &\textbf{76.79}	    &  {\bf 7.23\%}	 &\textbf{18.43}        &{\bf 138.83}       & {\bf 25.59}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.2: Europe setting} \label{tab:case3.2Europe}
\end{table}
%3. case World 
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c}
        \hline
         \textbf{No of}       &\textbf{Total}      & \textbf{Stale}  & \textbf{Genuine} & \textbf{Stale}  &\textbf{Mean}          &{\bf Avg. }      & {\bf Throughput} \\
		 \textbf{Miners/}     &\textbf{Blocks}     & \textbf{Blocks} & \textbf{Blocks}  & \textbf{Rate}   &\textbf{Prop.}         &\textbf{Traffic} & {\bf (TX/s)} \\    
         \textbf{Total}       & 				   &   			     & 			        &                 &\textbf{Delay(s)}	  & \textbf{(Kbps)} & \\
         \hline
         \textbf{6/83}        & \textbf{94.52}    &\textbf{4.3}      &\textbf{90.22}	&  {\bf 4.54\%}	 &\textbf{12.48}        &{\bf 146.97}        & {\bf 30.73}\\
         \hline
         \textbf{12/166}    & \textbf{95.17}      &\textbf{8.24}	 &\textbf{86.93}	&  {\bf 8.65\%}	 &\textbf{11.91}        &{\bf 142.04}        & {\bf 28.97}\\
         \hline         
         \textbf{18/250}    & \textbf{92.88}      &\textbf{7.2}	     &\textbf{85.68}	&  {\bf 7.75\%}	 &\textbf{11}           &{\bf 138.45}        & {\bf 28.56}\\
         \hline 
         \textbf{36/500}    & \textbf{99.83}     &\textbf{10.96}	 &\textbf{88.87}	&  {\bf 10.97\%} &\textbf{17.72}        &{\bf 150.56}         & {\bf 29.62}\\
         \hline  
         \textbf{54/750}    & \textbf{90.18}     &\textbf{7.46}	     &\textbf{82.72}	&  {\bf 8.27\%}	 &\textbf{19.45}        &{\bf 137.48}       & {\bf 27.57}\\
         \hline 
         \textbf{72/1000}   & \textbf{92.28}    &\textbf{11.44}	   &\textbf{80.84}	  &  {\bf 12.39\%}	 &\textbf{18.38}        &{\bf 140.83}       & {\bf 26.94}\\
         \hline 
         \textbf{90/1250}   & \textbf{82.03}    &\textbf{10.86}	   &\textbf{71.17}	  &  {\bf 13.24\%}	 &\textbf{20.01}        &{\bf 139.55}       & {\bf 23.72}\\
         \hline       
    \end{tabular}
\caption{Evaluation 3.2: World setting} \label{tab:case3.2World}
\end{table}
\fi








\iffalse
\begin{table*}  
\centering
\setlength{\tabcolsep}{10pt}
\begin{tabular} {|ccc|} %{ |l *{6}{D{.}{.}{4}}} {|ccc|cc|cc|}
\toprule
\textbf{Aspects} &  \textbf{Vectors} & \textbf{Metrics} \\

\cmidrule(lr){1-1} \cmidrule(lr){2-2}  \cmidrule(lr){3-3} 
%\midrule
\textbf{\textit{Scalability}} 	    &$\diamond$ No of devices		     		         & $\ast$ Maximum no of IoT devices as blockchain peers \\
\textbf{}		   			  		&$\diamond$ Transaction throughput of the system    & $\ast$ Maximum transaction throughput of blockchain system\\
\hline
\textbf{\textit{Security}} 	        &$\diamond$ Total amount of work     & $\ast$ Maximum result of the genuine block multiplied by  \\
\textbf{}		    		        &put to the blockchain				 &  difficulty of the PoW puzzle to generate a block\\
\hline
\textbf{\textit{Consensus}} 	&$\diamond$ Block propagation   &$\ast$ $\displaystyle\frac{\mbox{mean block propagation delay}}{\mbox{block generation interval}}$ $\leq$ 1 \\
\hline
\textbf{\textit{Resource}} 		&$\diamond$ Memory, processor, storage consumption  & $\ast$ Minimum difficulty of the PoW puzzle\\
\textbf{\textit{Consumption}}		&$\diamond$ Bandwidth consumption             & $\ast$ Average network traffic of a device $\leq$ 500 Kbps \\
\hline
\textbf{\textit{Efficiency }} &$\diamond$ Waste of energy and resources	 & $\ast$ Stale block generation rate  $\approx$ 1\%\\
\bottomrule             
\end{tabular}
\caption{IoT - Blockchain Integration Metrics} \label{tab:metrics} 
\end{table*}
\fi


%Therefore maximum number of IoT devices should be peers of the blockchain and  maximum transaction throughput should be achieved in the blockchain system.
%This is a very important issue that affects blockchain systems.
%For example, today's popular blockchain system Bitcoin having scalability issues due to low transaction throughput\footnote{$wikipedia.org/wiki/Bitcoin_scalability_problem$}, which led part of Bitcoin community to fork the Bitcoin blockchain and generate another coin named Bitcoin Cash\footnote{$en.wikipedia.org/wiki/Bitcoin_Cash$}, to process more transactions.

%Building on these aspects, we further specified vectors of these aspects, such as scalability - number of devices and transaction throughput.
%Finally, we specified IoT- blockchain integration metrics by considering needs and capabilities of IoT domain, that are presented in the Table \ref{tab:metrics}.



%\textbf{Novelty and value of the proposed architecture}
%\begin{itemize}
%\item Exploits decentralization, security and accountability features of blockchain technology on IoT domain. 
%\item Proposes multiple blockchains rather than a unique blockchain to offer better scalability and performance.
%\item Decreases in storage, memory and CPU overhead given by blockchain protocol to the IoT device . 
%\end{itemize}






%\textbf{Example scenario} Let us discuss an example IoT use case scenario with multiple blockchain architecture.  
%As discussed in \cite{supplyChainNetwork}, the supply chain network structure consists of many member firms and complex links between these firms, associated to the generation of a product, output value. Today's supply-chain systems have native needs like sustainability, transparency, visibility and need of decentralized infrastructure make supply chain scenario are good use case for integration of IoT and blockchain technologies. As the supply chain networks continues to grow in complexity, both in terms of the levels in the supply chain and the number of linkages, it can easily become untraceable \cite{complexSupplyChain}. 
%By integration of blockchain technology, immutable, shared and distributed nature of blockchains and permanent digital records of transactions may solve traceability issue and offer better provenance\footnote{www.wired.co.uk/article/wired-retail-2015}. 
%Given this, with the help of IoT technology using blockchain technology as background, enterprises may improve operational processes and reduce costs and risks due to transparency, traceability and adaptability. 
%In such a scenario, IoT devices  generation, transfer and update of products will be triggered by transactions of blockchain nodes. 
%Let us consider a very complex supply chain network, involving many suppliers and products, that generations massive amount of transactions.  
%Such a system will require high throughput of transaction execution, which might be a problem for a system of IoT devices with restricted resources. 
%Increasing number of blockchains, thus decreasing devices participating to the blockchain network offers to have better throughput and lower network latency of the system. 


%As an example, Bitcoin uses \textit{Simplified Payment Verification (SPV)}\footnote{www.bitcoin.org/en/developer-guide\#simplified-payment-verification-spv} protocol for light clients, where SPV protocol allows thin clients only to download block headers rather than all blocks to verify that particular transaction is indeed part of the block. In section \ref{sec:performanceLight}, we have tested and discussed about performance of the light clients of Bitcoin protocol, and we have showed that such methodology significantly decreases amount of resources used by the blockchain protocol.
%for such problems by transaction throughput needed. We want to underline that, design of such system is application specific, and capabilities of IoT devices and transaction volume between subset of devices plays a crucial role for design.
%\cite{supplyChainNetwork}
%So, instead of designing a new blockchain from scratch, our suggestion is to develop distributed applications for the IoT on top of the Bitcoin or another secure and stable blockchain. This can be done by leveraging a layered architecture, like the one proposed in Blockstack [40]. In this solution, the additional functionalities of the application are defined in another layer on top of the blockchain. Moreover, the blockchain is hidden at the application level, so low- performance IoT devices are not required to compute the PoW. 
%Relations: We could make use of Smart Contracts to set the rules on how the devices relate (collaborate) with each other. This way no intermediary is needed when any internet connected device wants to buy information or hire services from any other device. Also this intelligent agents may be able to negotiate prices (and discover new providers) to function autonomously.
%Payments. Payments, micro-payments and nano-payments between machines. Even bartering services could be possible. Hours of service of a particular device could be exchange for information provided for another one. Micropayment channels and nanopayments could be really useful in this scenario.
%We presume that for successful integration of blockchain technology into the IoT domain and to have more scalable architectural model, it is needed to exploit a multiple blockchain approach.
%Clearly, we need a backbone multi blockchain framework for proposed architecture. In section \ref{sec:systems}, discussion about multi-chain framework Polkadot, and its mechanisms and stakeholders has been given. 
%Applying IoT technology can optimize and affect whole supply-chain management paradigm by enabling  many features.
%In supply-chain systems, products have very complex and global manufacturing.
%As an example, IoT devices may be used as tools of asset tracking, which gives companies a way to improve their logistics operations and supply chain. Similarly, IoT technology allows to inventory and fleet management.
%IoT devices that capture finely granular real-time data about product and environment characteristics as well as location and timestamps throughout the supply chain, will be a solution for lack of a digital footprint, and improve provenance \cite{kim2016towards}.
%complexity of interactions between upstream and downstream linkages.
%Therefore let us discuss briefly about light client concept used by today's popular blockchain systems Bitcoin and Ethereum, since their light client ideology has effected our data structure design. Let us present \textit{Light Client Protocol (LCP)\footnote{\label{note1}www.github.com/ethereum/wiki/wiki/Light-client-protocol}} of Ethereum and \textit{Simplified Payment Verification (SPV)}\footnote{www.bitcoin.org/en/developer-guide\#simplified-payment-verification-spv} protocol of Bitcoin.
% Presentation of Ethereum's light client methods 
%LCP of Ethereum allows users in low capacity environments to maintain high-security assurance of verifying transaction executions and learning states of accounts without maintaining fully-synchronised database of Ethereum blockchain. In general, light client can be considered as a client that downloads block headers by default, and verifies only a small portion of what needs to be verified (transaction, state etc.), using a distributed hash table as a database for trie nodes in place of its local hard drive. In order to check whether a transaction is processed, light clients asks for block number including the particular transaction aimed to be verified and \textit{merkle path} of the merkle patricia tree including transaction. 
% Presentation of Bitcoin's light client methods 
%SPV protocol of Bitcoin allows thin clients only to download block headers rather than all blocks to verify that particular transaction is indeed part of the block. In SPV, client verifies that difficulty is high enough and block heads connected correctly simply checking previous hashes of each block and to verify transaction is indeed that particular block, they connect to a full node containing synchronized copy of blockchain, to get list of transactions in merkle path of the transaction to be verified. 
%Let us assume that supply chain scenario of a product consists involvement of many different products generated by different firms, each of which has its own lifecycle, which may include process phases of multiple companies and stakeholders.
%Let us present the potenatial challenges that may arise while IoT and blockchain integra
%\textbf{Multiple blockchain system} We propose a general multi-blockchain architecture, which assumes different blockchain protocols are able to send transactions to each other securely without losing accountability. ere are different proposals on multi-blockchain systems in literature like \cite{polkadot, cosmos,ethereumMauve}. In Section \ref{sec:architecture}, we discuss our expectations from such multi blockchain framework. Even though such back-end system is not in the scope of this paper, let us discuss an example of such multi-blockchain system, namely Polkadot. 
% \footnote{In Section \ref{sec:background} we briefly discussed an example heterogeneous multi blockchain project Polkadot} abilities to cooperate with each other, 
%We would like to underline that, our aim is not proposing an architecture for a specific IoT application, we do not focus on device structure, services or communication layers etc., but rather we propose methodology for the best integration of blockchain technology into IoT domain.
%The main motivation of the proposed architecture is providing 
%We assume blockchains used in proposed architecture will be able to communicate, and share transactions with each other.
%The proposed architectural model adjusts blockchain technology as a backbone technology, 
%\textbf{Architecture design principle}  
%Proposed architecture exploits foundational properties blockchain technology to build more robust and secure IoT systems, as discussed in Section \ref{sec:motivation}. In designing proposed architecture to generate a flexible architecture for IoT, we have considered diversity of the IoT ecosystem (e.g. device capabilities, application scenarios). Indeed, having common assumptions about IoT devices and application scenarios, and generating one size fits all design is not realistic for IoT domain. Therefore, we strongly believe that from architectural perspective being as general as possible is a must and protocol specifications of blockchains, like consensus protocols, should not be defined under strict terms. As an example, if we consider blockchain consensus protocols, there are always trade-offs between different protocols as discussed in \cite{quest}, and there is no optimal consensus solution that is best for every use case. As such, our core design principle is based on in this motivation. 
%-- IoT is mentioned as a possible field in which each device is identified by a public key to interact with other devices through the blockchain.
%Let us briefly discuss main features and what we expect from such multi blockchain back-end framework to be used as backbone framework for proposed multi  blockchain architecture. 
%Foremost important objective of such framework is processing inter-blockchain transactions with proved correctness and guaranteed overall system integrity in a secure way. 
%Firstly inter-chain transaction should at blockchain it is originated. If a transaction is not valid in its local blockchain, then the multiple blockchain framework should not accept it in the first place. 
%We presume, most likely such multiple blockchain framework will have its own blockchain to enhance security and integrity of the overall system.  
%Secondly, in order to have overall system integrity, a copy of each inter-chain transaction must be kept by the multiple blockchain framework, presumably in its blockchain, and integrity of the such transactions has to be ensured. 
%Finally, sending transactions from one blockchain to another have to be performed 
%There are different proposals on multi-blockchain systems in literature like \cite{polkadot, cosmos, ethereumMauve}. 
%\textbf{Connection of blockchains} Multiple blockchains will be able to send transactions to each other via inter-chain transactions, which will enable system to cooperate as like unique blockchain with increased interoperability.
%By exploiting inter-chain transactions, different application scenarios using their own local blockchain can cooperate with each other, without compromising accountability provided by blockchain technology.
%By recording inter-chain transactions, most likely in multiple blockchain framework's own blockchain, a process involving many participants from different blockchains will have accountability.
%may generate bottleneck for the system if they fully participate in blockchain protocols like consensus and block generation. 
%Proposed architecture aims to be suitable of complex systems including many heterogeneous IoT devices. 
%As such, for IoT devices with low capabilities, we propose to use of different roles of blockchain peers, as \textit{full peers} and \textit{thin clients} similar to Bitcoin\footnote{www.en.bitcoin.it/wiki/Clients}.
%There are two main scalability issues. The first is that, when the number of transactions grows, the blockchain increases in size, and it becomes expensive to store it, especially for IoT devices with limited resources.
%The second issue is the low throughput of transactions - a typical issue of the Bitcoin blockchain, which we did not find in the papers but is largely discussed within the Bitcoin community.



%(Even though, participants of the public blockchains can form up groups to take action together, such as mining pools of Bitcoin and Ethereum, which in some sense, may decrease the overall decentralization of the blockchain system).
%Another option is adoption to the existing public blockchains, such as Bitcoin or Ethereum.
%However adoption to the existing public blockchains is also not feasible, due to transaction fees and scalability issues considering number of devices and their capabilities..

%Such devices should be given with easier roles to perform like generating and sending transactions or checking block headers.
%However, they should not participate in the complex tasks such as block generation and consensus processes.

%Even though bigger blocks cause higher stale block generation rates, transaction throughput increases as they include more transactions.
%For example, in 1 minute block generation interval setting, with 100 KB blocks transaction throughput per second is 6.6 whereas with 10 MB block size, transaction throughput is 197.53, which is the highest transaction throughput we have observed in our evaluations.
%Moreover, long block propagation delays implies longer time to achieve consensus on the longest blockchain. 
%In our evaluations, we have observed observe this by comparing number of genuine blocks that have been generated in our evaluations in fixed time interval of 100 minutes.
%For example in 1 minute block generation interval setting, with 100 KB block size stale block rate is 0\% and number of genuine blocks is 99, whereas with 10 MB block size stale block rate is 35.07\% and number of genuine blocks is 26.93. 
%However, we have to note that, in case of higher network latencies and lower bandwidth capabilities, stale block rates will be higher.
%In such a case, bigger blocks will not imply higher transaction throughputs.
% Block generation interval: Block propagation time:  STALE RATES / Throughput  
%Similar to block sizes, also block generation intervals impact block propagation times, stale block rates, time required to achieve consensus and throughput.
%In IoT devices have to check and propagate blocks faster with shorter block generation intervals.
%However as IoT devices have limited resources and bandwidth capabilities, they may fail to finish block checking and propagation in short time intervals.   
%Indeed, this causes increase in the mean block propagation delays, as new generated blocks wait longer to be propagated across the network between IoT devices.
%For example with 500 KB block size, mean block propagation delay in 10 second block generation interval setting is 314.08 seconds, whereas it is 6.89 seconds in 5 minutes block generation interval setting.
%As expected, this in turn increases stale block rates of the system.
%For example with 500 KB block size, in 5 minute block generation interval setting stale block rate is 0\%,  whereas for 5 seconds block generation interval setting it is 45.96\%.
%However, for very small block sizes, short block generation interval settings do not increase stale block rates.
%For example with 10 KB and 50 KB block sizes, stale block rates are always lower than 1\%.
%In which, we have observed that, block generation interval and block sizes are not independent from each other and they should be set with respect to their values.
%As such, for big block sizes (e.g. 5 MB, 10 MB), long block generation intervals (e.g. 5 minutes, 10 minutes) have to be selected. 
%Whereas, for shorter block generation intervals (e.g. 10 seconds, 5 seconds), smaller blocks have to be used in the system (e.g. 10 KB or 50 KB).
%To conclude, block generation intervals have to be long enough regarding bandwidth capabilities of the IoT devices and block sizes.
%For IoT settings, using very big blocks are not suitable (e.g. 5 MB, 10 MB), as systems that have been configured with big blocks have long mean block propagation delay and achieve consensus later. 
%Thus, they have high stale block block generation rates and low transaction throughputs.
%On the other hand, very short block generation interval settings (e.g. 5 seconds, 10 seconds) result with long block propagation delay, high stale block generation rates and thus low transaction throughputs.
%As stale blocks are not part of the blockchain, they are lost efforts and waster of devices' resources and energy.
%Particularly, as the Netherlands setting has the shortest network latencies among nodes, best transaction throughput of 110.44 transaction per second have been observed in the Netherlands setting. 
%Higher block generation frequencies (e.g. 10 seconds, 5 seconds) increases stale block rates, thus, transaction throughputs are lower.  
%Our main inference from our observations on experiment results is; decreasing network latency among nodes is highly beneficial for blockchain adoption to IoT domain. 
%Indeed, having less network latency among nodes results with lower stale blocks and thus better transaction throughputs and faster consensus. 
%Particularly, a miner IoT device may not be aware of a new block that has been mined and published by another device due to long block propagation delays.
%In such a case, a miner IoT device would continue to mine and publish a new block by building on his view of the blockchain. 
%If we assume majority of the devices are aware of the new block and have already updated their local blockchains, the block published by unaware miner will be a stale block.
%However, stale blocks means lost efforts of the devices, thus, we prefer to have less stale blocks in the blockchain systems.
%We have observed the same behavior in evaluations results, that is, evaluations with
%Therefore long block propagation delays increase stale block rate.
%This means, the Netherlands settings have the lowest stale block rates in all evaluation cases with different block generation intervals.
%Transaction throughput of the system depends on number of genuine blocks, in which, low stale block rates imply high transaction throughput.   
%Therefore, the Netherlands setting have the highest transaction throughputs in all evaluation cases.
%Another important aspect effected by longer block propagation delays is the time required to achieve consensus, as its take longer time for the majority of the devices to have the same view of the blockchain.
%We can observe this by comparing number of genuine blocks that have been generated in our evaluations, as it presents the number of blocks that majority of the devices have consensed on fixed time interval (i.e. 100 minutes).
%Indeed, in our evaluation results, the highest number of genuine blocks have been observed in the Netherlands settings, for every block generation interval case.
%For example, for the 10 seconds block generation interval case, number of genuine block generated in the Netherlands setting is 133.23, whereas for %Europe setting it is 97.40. and for World setting it is 83.58.
%To conclude, shorter network latencies between IoT devices led blockchain system to have consensus faster, have lower stale block rates and higher transaction throughput. 
\iffalse
\begin{table*}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
         \textbf{Block  } & {\bf Total } &  \textbf{Stale} & \textbf{Genuine}  &{\bf Stale}  &{\bf Mean}    &{\bf Total}   &{\bf Average }  & {\bf Throughput} \\
		 \textbf{Size}    &\textbf{Blocks}& \textbf{Blocks} & \textbf{Blocks}  &\textbf{Rate}&\textbf{delay}&\textbf{Traffic} &\textbf{Traffic} & \\ 
        \hline
         \textbf{10 MB} 	 & {\bf 139.06} 		& \textbf{101.79} 		 &{\bf 37.27}  			  &  {\bf 73.19\%}	 & {\bf 2342.38s}   & \textbf{3252.38s}	 &{\bf 3252.38s}  & {\bf 248.46 TX/s}  \\
        \hline
         \textbf{5 MB}		 & {\bf 176.25}		    & \textbf{134.46}		 &{\bf 41.79}  			  &  {\bf 76.20\%} 	 & {\bf 2314.44s}   & \textbf{3028.62s}	 &{\bf 3252.38s}  & {\bf 139.30 TX/s}  \\
        \hline
         \textbf{1 MB}		 & {\bf 322.39} 		& \textbf{247.72} 		 &{\bf 74.67}     		  &  {\bf 76.83\%} 	 & {\bf 1752.36s}   & \textbf{2499.64s}  &{\bf 3252.38s} & {\bf 49.78 TX/s} \\
        \hline
         \textbf{500 KB} 	 & {\bf 426.35}         & \textbf{327.40} 	     &{\bf 98.95}             &  {\bf 76.79\%}   & {\bf 1596.04s}   & \textbf{2360.82s}  &{\bf 3252.38s}   & {\bf 32.98 TX/s}\\
        \hline
         \textbf{100 KB}     & {\bf ...}         &\textbf{}         &{\bf }             &  {\bf \%}   & {\bf s}   & \textbf{s}  &{\bf GB}   & {\bf TX/s} \\
        \hline 
         \textbf{50 KB} 	 & {\bf ...}         &\textbf{}         &{\bf }             &  {\bf \%}   & {\bf s}   & \textbf{s}  &{\bf GB}   & {\bf TX/s} \\
        \hline      
         \textbf{10 KB}       &{\bf 5361.31}        &\textbf{54.45}           &{\bf 5306.86}          &  {\bf 1.01\%}     & {\bf 3.00s}     & \textbf{0.49s}  &{\bf 3252.38s}   & {\bf 35.37 TX/s}  \\
        \hline    
    \end{tabular}
\caption{1 second block generation interval setting} \label{tab:1sec}
\end{table*}
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
          \textbf{Settings} & \textbf{Case \rom{1}} & \textbf{Case \rom{2}} & \textbf{Case \rom{3}} & \textbf{Case \rom{4}} & \textbf{Case \rom{5}} & \textbf{Case \rom{6}} & \textbf{Case \rom{7}}\\ 
        \hline
          \textbf{Node} 	  & \textbf{6 M} 		  & \textbf{12 M}		  & \textbf{18 M} 		  & \textbf{36 M} 		  & \textbf{54 M} 		  & \textbf{72 M} 		  & \textbf{90 M} \\
          \textbf{Setup}	  & \textbf{83 T} 		  & \textbf{166 T} 	   	  & \textbf{250 T} 		  & \textbf{500 T} 		  & \textbf{750 T}		  & \textbf{1000 T} 	  & \textbf{1250 T} \\
         \hline
          \textbf{Hash Power} & \textbf{1H} 	  	  & {\bf 2H}		 	  & {\bf 3H} 		      & \textbf{6H} 		  &{\bf 9H}  	 		  &{\bf 12H}	   		  &{\bf 15H}   \\
       \hline
       \textbf{Block }   & & & & & & &\\
        \textbf{Generation } &\textbf{3 mins}		& {\bf 1.5 min}	 	      & {\bf 1 min}	 		  &\textbf{30 secs}  	   &{\bf 20 secs}  		  &{\bf 15 secs} 		  &{\bf 12 secs}  \\		
        \textbf{Interval}& & & & & & &\\
        \hline
    \end{tabular}
\caption{Hash power experiments settings} \label{tab:caseSettings}
\end{table}
\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
          \textbf{Settings}   & \textbf{Case \rom{1}} & \textbf{Case \rom{2}} & \textbf{Case \rom{3}} & \textbf{Case \rom{4}} & \textbf{Case \rom{5}} & \textbf{Case \rom{6}} & \textbf{Case \rom{7}}\\ 
        \hline
          \textbf{Netherlands}& \textbf{6 M} 		  & \textbf{12 M}		  & \textbf{18 M} 		  & \textbf{36 M} 		  & \textbf{54 M} 		  & \textbf{72 M} 		  & \textbf{90 M} \\
         \hline
          \textbf{Europe}     & \textbf{1H} 	  	  & {\bf 2H}		 	  & {\bf 3H} 		      & \textbf{6H} 		  &{\bf 9H}  	 		  &{\bf 12H}	   		  &{\bf 15H}   \\
       \hline
        \textbf{World}        &\textbf{3 mins}		 & {\bf 1.5 min}	 	      & {\bf 1 min}	 		  &\textbf{30 secs}  	   &{\bf 20 secs}  		  &{\bf 15 secs} 		  &{\bf 12 secs}  \\		
        \hline
    \end{tabular}
\caption{Hash power experiments settings} \label{tab:caseSettings}
\end{table}
\begin{figure} [H]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/chart2.png}
	\caption{ Cost - difficulty relation \label{fig:cost2}}
\end{figure}
\fi


\subsection{Req Findings}\ref{sec:reqFindings}
%Let us exploit the Bitcoin simulator presented in \ref{sec:simulatorSettings} to test transaction throughput of a proposed setting and unique blockchain setting, in fixed 500 Kb block size setting with regards to blockchain-IoT integration metrics presented in Section \ref{sec:metrics}.
%For example by having 250 IoT devices in \textit{the Netherlands} setting, the shortest block generation interval setting is 30 seconds and number of transactions per device in a minute is 12.
%However, as a unique blockchain setting by having 2000 IoT devices in \textit{World} setting, the shortest block generation interval setting that satisfies blockchain-IoT integration metrics given in Section \ref{sec:metrics} is 12 minutes and number of transactions per device in a minute is 0.1.
%In proposed setting, devices in different subgroups are able to send transactions to each other.
%Therefore, dividing IoT devices into subgroups do not cause to decrease number of devices participating in the system.
%In overall system, multiple blockchains contain same amount of devices a unique blockchain, with much lower stale block generations rates and block propagation delays (as evaluated in Section \ref{sec:reqEva1}, \ref{sec:reqEva2} and \ref{sec:reqEva3}).


%Several features of blockchain technology and characteristics of IoT domain should be taken into consideration to enable blockchain technology into the IoT domain.
%To evaluate and analyze such features, we specified a set of integration metrics that is presented in Section \ref{sec:metrics}.
%We have evaluated many features of blockchain IoT integration by exploiting the Bitcoin simulator presented in Section \ref{sec:simulatorSettings} and referring to the blockchain IoT integration metrics.




PERFORMANCE

%We recall that in proposed architecture three roles have been defined for IoT devices as: outsider devices, light peer devices and full peer devices.
%Light and full peer devices directly peers of the blockchain network, thus blockchain operations affect their performance.
%However, outsider devices aren't peers of the blockchain and they do not perform blockchain operations, thus being part of a blockchain network doesn't affect their performance.
%Given that, we evaluate performance of the light peer and full peer devices.
%To measure and monitor performance of 

%In our DoS attack scenario, a full peer device is the victim device, and it is attacked by 10 (DoS scenario \rom{1}) and 20 (DoS scenario \rom{2}) light peer devices by sending many transactions.
%This DoS attack aims to overwhelm IoT device by increasing it's CPU usage and bandwidth consumption as it has to check correctness of each transaction.
%We generated two DoS scenarios as DoS scenario \rom{1} with 10 attacker devices and \rom{2} with 10 attacker devices.
%For both of evaluation cases we performed to attack for 45 minutes.
%In DoS scenario \rom{1} 83100 transactions sent by attacker devices with an average of 8100 transactions per attacker. 
%Whereas, in DoS scenario \rom{2} 108960 transactions sent by attacker devices with an average of 5448 transactions per attacker. 
%Decrease in number of transaction send by an attacker device decrease in DoS scenario \rom{2} due to overwhelm of the victim IoT device.




%where in total 65000 transactions with one input (attacker node's account address) and one output address, sent to the victim device. 
%Due limited resources of light peer devices, light peer devices run Alpine Linux operating system\footnote{alpinelinux.org} version 3.6.0, that is a lightweight Linux o.s. distribution that only requires around 5 MB of storage. 
%Whereas, light peer devices set up with 120 MB of RAM, and their CPU usage is limited to 2\% of one core of Intel Core i7 2.70 GHz CPU. 
%We have evaluated the effect of size of the blockchain to resource usage of IoT devices acting as full peers of blockchain network by using device configuration settings previously given in Section \ref{sec:emulationStructure}. 
%noktalar arasi direk 5.3 Eva 2 ye gitcek
%First, in order to test performance of the full peers and scalability of the proposed architecture, we have emulated 200 IoT devices on IBM Power 8 server. 
%IoT devices configured with 512 MB of RAM (memory swap is disabled) and 5\% of a single Power8 CPU\footnote{https://www-01.ibm.com/common/ssi/cgi-bin/ssialias?htmlfid=POB03046USEN}, which has 3.5 GHz clock rate. 
\iffalse
\begin{figure*} 
    \centering
  \subfloat[20 nodes]{%      
     \includegraphics[width=0.25\linewidth]{figures/CPU_Utilization-10lu.png}}
  	  \label{1a}\hfill
  \subfloat[40 nodes]{%
      \includegraphics[width=0.25\linewidth]{figures/CPU_Utilization-20li.png}}
    \label{1b}\hfill
  \subfloat[100 nodes]{%
      \includegraphics[width=0.25\linewidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}}
     \label{1c}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.25\linewidth]{figures/Total_Ethernet_Read_and_Write-20li.png}}
     \label{1d} 
  \caption{(a), (b), (c), (d).}
  \label{fig:CpuUtil} 
\end{figure*}
\fi

\iffalse
\begin{figure} 
    \centering
  \subfloat[100 nodes]{%
     \includegraphics[width=0.5\linewidth]{figures/CPU_Utilization-10lu.png}}
     \label{1d}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/CPU_Utilization-20li.png}}
     \label{1e} 
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure}

\begin{figure} 
    \centering
  \subfloat[100 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}}
     \label{1d}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Total_Ethernet_Read_and_Write-20li.png}}
     \label{1e} 
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure}



 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}
	\caption{Full peer ETH Sce \rom{1}} \label{fig:architecture}
\end{figure}


 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figures/Total_Ethernet_Read_and_Write-20li.png}
	\caption{Full peer ETH Sce \rom{2}} \label{fig:architecture}
\end{figure}

 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figures/CPU_Utilization-10lu.png}
	\caption{Full peer 10lu} \label{fig:architecture}
\end{figure}


 \begin{figure} [h] 
	\centering
	\includegraphics[width=0.5\textwidth]{figures/CPU_Utilization-20li.png}
	\caption{Full peer 20li} \label{fig:architecture}
\end{figure}


\fi

\iffalse
\begin{figure} 
    \centering
  \subfloat[100 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Lightcpu.png}}
     \label{1d}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Lighteth0.png}}
     \label{1e} 
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure}
\fi

\iffalse
% \begin{figure} [h] 
%	\centering
%	\includegraphics[height=50mm]{figures/Lighteth0.png}
%	\caption{Light peer ETH} \label{fig:architecture}
%\end{figure}


 \begin{figure} [h] 
	\centering
	\includegraphics[height=50mm]{figures/Lightcpu.png}
	\caption{Light peer CPU} \label{fig:architecture}
\end{figure}
\fi

\iffalse
\begin{figure} 
    \centering
  \subfloat[100 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}}
     \label{1d}\hfill
  \subfloat[200 nodes]{%
      \includegraphics[width=0.5\linewidth]{figures/Total_Ethernet_Read_and_Write-20li.png}}
     \label{1e} 
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure}
\fi

\iffalse
  \subfloat[Full Peer  Network]{%
      \includegraphics[width=0.33\linewidth]{figures/Total_Ethernet_Read_and_Write-10lu.png}}
     \label{1d}\hfill
  \subfloat[Full Peer Sce \rom{2} Network]{%
      \includegraphics[width=0.33\linewidth]{figures/Total_Ethernet_Read_and_Write-20li.png}}
     \label{1e} 
\fi


\iffalse
\begin{figure*} 
    \centering
  \subfloat[Light Peer CPU CPU]{%
      \includegraphics[width=0.33\linewidth]{figures/Lightcpu.png}}
     \label{c} 
  \subfloat[Full Peer Sce \rom{1} CPU]{%
     \includegraphics[width=0.33\linewidth]{figures/CPU_Utilization-10lu.png}}
     \label{b}\hfill
  \subfloat[Full Peer Sce \rom{1} CPU]{%
      \includegraphics[width=0.33\linewidth]{figures/CPU_Utilization-20li.png}}
     \label{c}      
  \caption{DENEME}
  \label{fig:lightPeer} 
\end{figure*}
\fi





%Scalability is the biggest challenge to overcome in adapting blockchain technology into the IoT domain.
%Optimal blockchain system should have high transaction throughput and maximum number of nodes should participate in the blockchain.
%Therefore, we go for a hybrid blockchain architecture, both containing PoW and BFT blockchains, as a solution for scalability problem of IoT domain.
%Particularly, first IoT devices divide into subgroups and form PoW blockchains, like as sharding of a unique blockchain that would contain all devices.


%Sharding PoW blockchains requires elaborate evaluation of scalability, performance and security aspects have to be considered carefully. 
%We propose blockchain-IoT integration metrics to achieve high performance and scalability.
%If sharding a PoW blockchain into multiple blockchains decrease amount of work that each new blockchain contains, than they are more vulnerable against threats target their integrity.
%Given, that we quantitatively evaluated effects of sharding. 
%Therefore, we go for a hybrid blockchain architecture containing PoW and BFT blockchains. 
%Two popular blockchain consensus models, namely PoW and BFT, provide effective solutions to the different parts of the scalability problem \cite{quest}. 
%Particularly, PoW based blockchains are able to scale to thousands of nodes and BFT based blockchains can achieve thousands of transaction throughput.



\iffalse
Improving the performance of PoW blockchains. Sompolinski and Zohar GHOST (Greedy Heaviest-Observed Sub-Tree) rule [55], which
basically resolves conflicts in a PoW blockchain by weighing the subtrees rooted in blocks rather than the longest (sub)chain rooted in given blocks. 
Although
GHOST is essentially a conflict-resolution strategy, it offers performance benefits
over the standard longest (heaviest) chain rule of Bitcoin, as it provides more
secure means of increasing the block frequency and the block size [55]. A variant
of the GHOST rule is actually implemented in the Ethereum blockchain [58],
although the GHOST-PoW performance has not yet been adequately stresstested
with high loads (in 2016, typical Ethereum throughput is fewer than
20,000 transactions per day, i.e., about 0.2 tx/s on average).5
\fi


\iffalse
Hyperledger in yeni konsepti vukolic in paper dan
a. The new architecture [1], termed Fabric V1
here, separates the execution of smart-contract transactions (in the sense of validating the
inputs and outputs of a program) from ordering transactions for avoiding conflicts (in the
sense of an atomic broadcast that ensures consistency). This has several advantages, including
better scalability, a separation of trust assumptions for transaction validation and ordering,
support for non-deterministic smart contracts, partitioning of smart-contract code and data
across nodes, and using modular consensus implementations [59].
\fi
%In addition to performing inter-chain transactions, blockchain connector framework contains and executes smart contracts for all sub-blockchains, that are self-executable programs in the blockchain\cite{szabo}.
%The reason to separate smart contracts in spe
%Quest: Indeed, a smart contract can be modeled as a state machine, and its consistent execution across multiple nodes in a distributed environment can be achieved using state machine replication.
%BFT based multiple blockchain connector framework perform inter-chain and smart contract transactions of sub-blockchains and able to perform thousands of transactions per second \cite{consensusWild}.
%.

==> DEPRECATEDbackground.tex <==

Mutual contacts graphs represents complex interaction networks, where nodes represent hosts (i.e. device IPs) and edges mimic their similarity with regards to their connections. 
%In case of a Botnet attempt on part of the IoT network, mutual contact graph will evolve quickly.
%In fact, devices will connect to botmasters and most likely botmaster will cut other connections of the infected devices to be harder to prevent infection detection as a strategy of stealthy botnet (cite stealthy- if its in the definition), like as in Mirai botnet \cite{mirai}.
%When IoT network is under a threat of a P2P botnet, it most likely will have different mutual contacts graph.
%Therefore, analyzing multiple mutual contacts graphs of the same network that are generated in different time steps may let us acquire better detection of evolving botnet attacks.

Let us first model the botnet detection problem in IoT.
This problem has two main characteristics.
%In order to detect botnets on a particular mutual contacts graph, we perform community behavior analysis.
%Second, due to stealthy nature of the P2P botnets, structure of the mutual contacts graph evolves with time.
%Requirements of such a problem perfectly matches with the novel problem of \textit{identification of evolving communities} in dynamic networks.
%Where, dynamic networks evolve with the time (i.e. vertice and edge sets differ in time), and they can be used to model the evolution of a system: nodes and edges are mutable, and their presence/absence impacts the community structure that includes them \cite{communityDiscoveryInDynamicNetworksSurvey}.
%This problem captures many interest among researchers and various methodologies have been proposed, such as: \cite{quantifyingSocialGroupEvolution, trackingEvolutionOfCommunitiesInDynamicSocialNetworks, eventBasedFrameworkForCharacterizingEvolutionaryBehaviorInteractionGraphs}.
%Fortunately, we can exploit blockchain data structure to find the key solution to this problem.





\section{PoW Blockchains Background}\label{sec:background}
In this section, we provide a brief background information on PoW blockchains.
%Blockchain refers to distributed database, a shared ledger, on a peer to peer network. 
%Novelty of the blockchain technology lies in its ability to achieve coordination and verification of individual activities carried out by different parties without a centralized authority or trusted third party \cite{blockchainTechnology}.


\textbf{Blockchain structure.} 
Transactions transfer information (i.e. data packets) between peers and they have unique identifiers, input data, and they are bundled into data chunks called blocks. 
Every block contains set of transactions, a timestamp, a reference to the preceding block, and an authenticated data structure (i.e. a merkle tree) from previous transactions, and forms the blockchain. 
Blockchains are peer to peer networks, and nodes are connected to other nodes as peers to share transactions and blocks. 
A copy of the blockchain is stored on every node in the network and these peers exchange the latest block information with each other to ensure that all of them have the same shared database.


\textbf{PoW - block generation.}
Blockchain nodes have to solve a cryptographic puzzle, Proof of Work (PoW), to be authorized to generate a new block.
In generating a new block, miners nodes confirm that new transactions are valid and consistent with former transactions before sealing them into blocks. 
Main duty of the PoW is preventing instant block creations to reduce conflicts such as double spending and sybil attacks. 
Indeed, attackers can't easily create many blocks to shape an alternative blockchain, however it is easy to confirm once it is created.
Blockchain nodes trying to generate a new block is called \textit{miners}, block generation process is called \textit{mining}, miner's mining ability is referred as \textit{mining power}.
In PoW blockchain, difficulty of the PoW puzzle is used regulate expected average block generation interval according to the total mining power of the miners in the blockchain network.
In particular, to have a fixed block generation interval, difficulty is increased when total mining power increases, and it is decreased when total mining power decreases.


\textbf{Block sharing.}
Miners share the new found block with its peers at the time of solving the PoW puzzle.
Nodes that have received the new block are responsible for checking the correctness of the block, and legitimacy of the transactions inside the block, ensuring that they have not been included in any other block previously, before adding blocks to their local blockchain and propagating to their peers. 
Adding new blocks to the blockchain increases total amount that blockchain contains, and thus it increases security of the blockchain against adversaries trying to alter it.


\textbf{Stale blocks.}
Blockchains may have forks due to malicious manipulations or propagation delays and longest fork remains as the agreed and valid blockchain branch\cite{blockchainSurvey}(to the rest of the paper we will refer blocks included to the blockchain as genuine blocks). 
In general, blocks in shorter forks do not included in the blockchain and they referred as \textit{stale blocks}\footnote{In Ethereum blockchain(ethereum.org) they are included to the blockchain as uncle blocks, however they do not count towards total difficulty of the blockchain \cite{onTheSecurityPoW}}.
Stale blocks do not contribute to the security of the blockchain and transactions in stale blocks considered as unprocessed by the network, thus stale blocks should be considered as lost of efforts.
%In this case, the rate of discarded blocks (known as the orphan rate or the fork rate) increases and the security of the protocol deteriorates. 




Blockchains can be categorized into two groups with regards to their consensus methodologies as \textit{Proof of Work (PoW)} and \textit{Byzantine Fault Tolerant (BFT)} blockchains.
In PoW-based blockchains, such as Bitcoin \cite{bitcoinNakamoto} and Ethereum \cite{ethereumYellowpaper}, peers have to solve a cryptographic puzzle as proof of their work in order to be authorized to generate a new block. 
PoW-based blockchains able to scale thousands of nodes in achieving consensus. 
On the other hand BFT-based blockchain protocols, such as Hyperledger \cite{hyperledger}, achieve consensus by state replication with assumption of limited number of faulty peers.
BFT-based blockchain protocols can achieve thousands of transactions throughput \cite{quest}.












\textbf{Why ML was not successful in intrusion detection - Taken from \cite{outsideTheClosedWorldOnUsingMLforNetIntrusionDetection}:} 
There is surprising imbalance between the extensive amount of research on machine learning-based anomaly detection pursued in the academic intrusion detection community, versus the lack of operational deployments of such systems. We argue that this discrepancy stems in large part from specifics of the problem domain that make it significantly harder to apply machine learning effectively than in many other areas of computer science where such schemes are used with greater success.
The domain-specific challenges include: (i) the need for outlier detection, while machine learning instead performs better at finding similarities; (ii) very high costs of classification errors, which render error rates as encountered in other domains unrealistic; (iii) a semantic gap between detection results and their operational interpretation; (iv) the enormous variability of benign traffic, making it difficult to find stable notions of normality; (v) significant challenges with performing sound evaluation; and (vi) the need to operate in an adversarial setting. While none of these render machine learning an inappropriate tool for intrusion detection, we deem their unfortunate combination in this domain as a primary reason for its lack of success.




Collaborative intrusion detection frameworks are widely adopted and deployed in various organizations due to the enhanced detection performance, but two major issues still
remain: data sharing and trust computation:
\begin{itemize}
\item Firstly, data sharing is a big challenge for collaborative detection, as not all parties want to share their information explicitly. For example, anomaly detection often employs machine learning techniques to build normal profiles, in which a classifier requires a large number of training items. Due to privacy concerns, some organizations are not willing to share their data, making the detection performance hard to optimize. 
\item Secondly, insider attacks are one big challenge for collaborative detection, which can greatly degrade the network security. Thus, how to effectively evaluate the trustworthiness of an IDS node is a challenge in a distributed and collaborative environment. For instance, with many collaborating parties, it is not an easy task to effectively measure their reputation levels.
\end{itemize}



%\textbf{Support this with the claims given in \cite{outsideTheClosedWorldOnUsingMLforNetIntrusionDetection}:}The fundamental goal of machine learning is to generalize beyond the examples in the training set. This is because, no matter how much data we have, it is very unlikely that we will see those exact examples again at test time \cite{fewUsefulThingsToKnowAboutML}.



Feature set of network traffic flow analysis.
Two sets of features: first standard set of features that can be observed by network traffic analyzers such as NetFlow\cite{netflow} that are presented in \cite{MLforIPtrafficFlowClassification}, and second is the enhanced set of features.....


Determining that a set of network connections from an enterprise network is truly benign is often impossible.
in \cite{mlForEncryptedMAlwareTrafClassification}, randomly change class of a fixed percentage of samples in part of data set, train the classifiers, and tested the classifiers on another part of the data.


FDR: In \cite{mlForEncryptedMAlwareTrafClassification}: Even moderately sized networks have tens-of-millions of network connections each day. Due to this scale, and the typical set of remediation actions that could be taken against a potentially malicious session, maintaining a low false positive rate is much more important than total accuracy. Figure 3 also reports the accuracy at a fixed .001\%, or 1-in-100,000, false discovery rate (FDR). This is the accuracy of the classier when it is only allowed one false positive for every 100,000 true positives.



\cite{mlForEncryptedMAlwareTrafClassification}: The network security domain poses a unique set of challenges, notably, the scale of the data, demand for very low false positive rates, evolving data streams and noisy class labels.
Although we found the random forest ensemble classifier to be the most robust for this problem domain, we demonstrated that the choice of features had much greater effect on performance. The enhanced feature set was created by augmenting a standard feature set used in domain with features identified by a domain expert and specifically tailored for encrypted network sessions.




In \cite{mlForEncryptedMAlwareTrafClassification}: The main difficulty against applying machine learning to the intrusion detection systems is achieving low false positive rates.
According to \cite{mlForEncryptedMAlwareTrafClassification}, there are two main reasons: first is the inaccurate ground truth as benign data may include malicious activity and malicious data may be lacking benign activities of malwares; and second is the non-stationary in network data as frequently communicated services may change. \\
-- Benim yorum: Yet we do not consider the second case for the low-level IoT devices, as standard application specific devices would communicate with similar services - with particular IP addresses.



Inaccurate ground truth (Can Adversarial machine learning be addressed?)
In \cite{mlForEncryptedMAlwareTrafClassification},: Adversarial machine learning promotes awareness of the types of attacks that can be perpetrated against machine learning system, and attempts to provide solutions in the form of robust data features and training algorithms.
Results on randomly changing label on data, also applicable to the situation in which an attacker has some influence over training data.



\textbf{Malware similarity Search:}
In \cite{learningCommPatternsMalwareDiscovHTTPs}: Keeping the trained anti-malware engines up to date is a challenging task as novel malware types emerge with unpredictable new forms.
Hence, once in a while network administrators could explore actual representative subsets of the proxy logs and manually investigate selected connections. In cases when an infected record is identified, an effective unsupervised recommendation method could help the administrators with the efficiency of the exploration process. One option is to employ the \textit{similarity search approach assuming that new malware types share similar communication patterns reflected in similar communication snapshots}. These similarities can provide clues for the detection of similar snapshots of novel types of malware, yet not registered (or misclassified) by present anti-malware engines. The similarity search can also provide an option to group communication descriptors based on additional properties (e.g., a contacted server). In order to perform similarity search in general, a standard approach is to employ a dissimilarity space (U, \textit{fi}), where U represents a descriptor universe and \textit{fi} : U × U $\rightarrow$ ${R_0+}$ represents a distance function.




==> DEPRECATEDrelated.tex <==
%done : 1)intro
\section{Related Work}\label{sec:related}
In recent years, vast amounts of work has been proposed as P2P botnet detection solutions.
Mainly, botnet detection methodologies can be categorized into two groups: host-based and network-based approaches. 
Host-based approaches require individual monitoring for all hosts, which is impractical for IoT domain.
Therefore, we focus on network-based approaches which we classify into two groups, discussed in what follows.


% : 2) Network traffic signature based
\textbf{Network traffic signature based approaches.} Literature offers many works that utilize network traffic behaviour classification for hosts, in order to identify whether they are benign or malicious, such as \cite{scalableSystemForStealthyP2PbotnetDetection, peershark, botminer, botdetector}.  
In \cite{scalableSystemForStealthyP2PbotnetDetection}, a statistical network traffic fingerprinting approach that is using unsupervised machine learning techniques to identify P2P activity and to group hosts participate in malicious P2P traffic.
PeerSark, proposed in \cite{peershark}, a port and protocol oblivious conversation-based approach to detect P2P botnet traffic is proposed. %NO DPI.
However in a dynamic network, such approaches are ineffective, as botnets can randomize their traffic, thus traffic signature will vary. 

%DPI-based traffic signature approaches.
Some other works rely on deep packet inspection techniques (DPI) in order to identify P2P botnets. 
For example, BotMiner proposed in \cite{botminer}, groups hosts that share similar communication patterns in performing malicious activities.
More recently, BotDetector proposed in \cite{botdetector},  leverages on DPI techniques to monitor information recorded on HTTP headers is proposed.
However, DPI based approaches are computationally expensive, and traffic flow encryption makes them methods ineffective.



% : 3) group and community behavior based
\textbf{Group and community behavior based approaches.}
In \cite{friendsOfAnEnemyMutualContacts}, a mutual contacts based approach that is based on network traffic flow of hosts is proposed to identify bots in a P2P network. However, this approach requires bot seeds/discovered bots in order to identify bots, which may not be available. 
Moreover, this approach is only limited to detect bots from previously known bot types.
PeerClean proposed in \cite{peercleanUnveilingP2PbotnetsThroughDynamicGroupBehaviorAnalysis}, performs group level behavior analysis on network flow traffic with SVM method. Similarly to the previous work, this approach is only limited to known bot types.
More recently, in \cite{peerhunter}, a network flow level community behaviour analysis is performed for P2P botnet detection.
Similar to our proposal, also this approach performs community analysis approach based on mutual contacts graph have been proposed.
However, it is a static approach, as it performs botnet detection once on collected network flow traffic data, yet AutoBotCatcher dynamically performs botnet detection on successive snapshots of the mutual contacts graph with the help of blockchain technology. 
%Moreover, it does not take any prevention measurements like AutoBotCatcher. 

%\textbf{-- Total number of citation can be reduced like 15}
%\textbf{-- Related work can be moved to introduction. }


% : 3) graph-based
%BOTGREP
%In \cite{botgrepFindingP2PbotsWithStructuredGraphAnalysis}, a communication graph structure based approach for P2P botnet detection.....
%. Botgrep [18] is a communication graph structure based botnet detection method, which can detect P2P botnets through localizing structured communication graphs. However, this method can only identify structured communication subgraphs, rather than ensure those subgraphs contain P2P botnets}

==> DEPRECATEDsecurity.tex <==
\iffalse
\textbf{Distributed Denial of Service Attacks (DDoS) \cite{botnetsInDDoSattacksSurvey}:} DDoS is a coordinated attack, generated by using many compromised hosts. An attacker initially identifies the vulnerabilities in a network to install malware programs on multiple machines to bring them under his control. Then the attacker uses these compromised hosts to send attack packets to the victim without the knowledge of the compromised hosts. Depending on the attack packet intensity and the number of hosts used for attacking, commensurate damage occurs in the victim network. \\ 
-- To launch an attack, an attacker generally follows four basic steps.
\begin{itemize}
\item information gathering to scan a network to find vulnerable hosts to use them later to launch an attack,
\item compromising the hosts to install malware or malicious programs in the compromised hosts (called zombies) so that they can be controlled only by the attacker,
\item launching the attack to command the zombies to send attack packets with specified intensities to the victim, and
\item cleaning up to remove all records or history files from memory.
\end{itemize}
-- Network security defenders must focus on protecting the network community from two basic types of DDoS attacks: (i) network/transport layer DDoS attacks and (ii) application layer DDoS attacks.\\
-- \textbf{Examples of Network/Transport Layer Attacks}: 
\begin{itemize}
\item In TCP SYN flooding, attack is generated by sending a large number of TCP SYN connection requests to overwhelm the server. To initiate the attack, the attacker creates packets with random source IP addresses for each packet, with the SYN flag set in each packet to open a new connection to the server from the spoofed IP addresses. On receipt, the victim responds to spoofed IP addresses and waits for confirmation that never arrives. As a consequence, victim’s connection table fills up waiting for replies and the server is not able to accept new connection any more.
\item In UDP flooding, due to its connectionless nature, the UDP protocol does not require any connection setup procedure to transfer data. To initiate this host-based flooding attack, the attacker sends a UDP packet to a random port on the victim system.
\item In ICMP flooding, which is also known as the ping-of-death attack
\end{itemize}
-- \textbf{Application Layer Attacks:} Application layer DDoS at- tacks generally target the HTTP protocol with an objective to exhaust limited resources available to Web services. Typically, such attacks are not trivial to identify because they look similar to legitimate traffic and the volume of traffic is also not too large. The three main reasons behind the difficulty in detecting this type of DDoS attack [12] are:
\begin{itemize}
\item (i) Obscurity, the use of legitimate TCP and UDP connections during the attack makes it difficult to distinguish it as illegitimate traffic. 
\item (ii) Efficiency, the need for fewer connections to launch an attack successfully makes it efficient.
\item (iii) Lethality, it can overwhelm resources of services quickly, resulting in denial of services regardless of the abilities of the hardware of the host.
\end{itemize}
-- \textbf{Examples of Application Layer Attacks}: 
\begin{itemize}
\item HTTP attacks: This type of application-based attacks usually occurs in three forms. (i) HTTP malformed attacks, (ii) HTTP request attacks, (iii) HTTP idle attacks.
%Request-Flooding Attacks: An attacker initiates these attacks by sending legitimate requests at a higher rate such as HTTP GET, HTTP POST and DNS queries to a server in order to overwhelm its session resources.  
\item DNS attacks: This application-based attack has four distinct sub-categories. (i) DNS query (or answer) malformed packet attacks, (ii) man-in-the-middle and DNS cache poisoning attacks, (iii) DNS amplification attacks, (iv) DNS dictionary attacks.
%Asymmetric Attacks: In these attacks, the attacker at- tempts to consume server resources such as CPU, memory or disk space by sending high workload requests at normal rates. The main goal of this attack is to consume such resources of a server in order to degrade the performance of services.
\item VoIP attacks: This category of application-based attacks also has four distinct sub-categories. (i) SIP invite flood attacks, (ii) SIP call setup request attacks, (iii) SIP malformed packet attacks, (iv) Real-time transport protocol (RTP) flood/quality of service (QoS) attacks.
%Repeated One-Shot Attacks: In this type of attack, an attacker sends a high workload request to many TCP sessions to degrade the performance of services. This type of attack is also considered an alternate (secret) way of executing request-flooding and asymmetric application- layer attacks.
\item SMTP attacks: There are two types of SMTP attacks. (i) SMTP error DoS, mailbox DoS (excessive email size) and SMTP mail flooding, (ii) SMTP buffer overflow attacks.
%Application-Exploit Attacks: To initiate these attacks, an attacker takes advantage of the vulnerabilities that arise during the running of an application on a target system. Here, the attacker attempts to cause a fault in the target’s operating system by running applications to gain control of one or more applications, the system or network. Some common examples of such attacks are Cross-site scripting (XSS), SQL injection (SQLIA), buffer overflows, scripting vulnerabilities, cookie poisoning and hidden- field manipulation. 
\end{itemize}
-- Botnet based attack launching technology is more serious in both network/transport layer as well as application layer DDoS attacks.\\
-- \textbf{To counter a botnet based attack}, it is essential for the network defender to know the malware code and enhancements that may have been applied to such code. In addition, the botnet architectures, topologies and protocols used for attacks should be carefully analyzed when developing a DDoS defense system.\\
-- Botnet-based \textbf{DDoS attacks are generally launched using three basic models} [13]: (i) agent handler model (ii) IRC botnet model and (iii) web-based model. \\
-- Internet Relay Chat (IRC), is a text-based chat system that organizes communication in channels. \textbf{IRC-based DDoS attacks} are now most popular because of their power to generate a huge volume of attack traffic instantly. Typically, this system installed with a bot can spread very fast and automatically exploit multiple vulnerabilities. After successful installation, a full backdoor generally resides on the system, including an IRC component to establish communication between the computer and a remote IRC server; this backdoor is controlled by the attacker. \\
-- To communicate with clients, the agents use an IRC communication channel as shown in Figure 8(b). The agents are communicated through IRC ports, which makes it difficult for the defender to trace DDoS command packets. 
\fi











